Solving Continual Combinatorial Selection via Deep Reinforcement Learning

We consider the Markov Decision Process (MDP) of selecting a subset of items at each step, termed the Select-MDP (S-MDP). The large state and action spaces of S-MDPs make them intractable to solve with typical reinforcement learning (RL) algorithms especially when the number of items is huge. In this paper, we present a deep RL algorithm to solve this issue by adopting the following key ideas. First, we convert the original S-MDP into an Iterative Select-MDP (IS-MDP), which is equivalent to the S-MDP in terms of optimal actions. IS-MDP decomposes a joint action of selecting K items simultaneously into K iterative selections resulting in the decrease of actions at the expense of an exponential increase of states. Second, we overcome this state space explo-sion by exploiting a special symmetry in IS-MDPs with novel weight shared Q-networks, which prov-ably maintain sufficient expressive power. Various experiments demonstrate that our approach works well even when the item space is large and that it scales to environments with item spaces different from those used in training.

==> einn_bk.tex <==
\section{Methods and Analysis}
\label{sec:Methods}

\begin{comment}
In this section, we explain how the proposed ideas in previous section
are utilized to construct our EINET and derive
a progressive algorithm to efficiently solve the select-MDP.
% In section~\ref{sec:greedy-select-dqn},
We first explain our greedy select-DQN algorithm with $K$ different Q-networks for greedy select-MDP with $K$ selections.
% In section~\ref{sec:EINET},
Then, we introduce our parameter shared neural network architecture for Q-networks, and provide mathematical analysis for optimality of the network.
% in section~\ref{sec:math-einet}.
Finally, some sharing techniques are proposed to make the algorithm more efficient.
% in section~\ref{sec:inter-intra}.
\end{comment}


In this section, we first present a symmetric property of IS-MDP, which is
referred to as {\em Equi-Invariance} (EI), and propose an efficient RL
algorithm to solve IS-MDP by constructing $K$ cascaded Q-networks with two-levels of parameter sharing. 

\subsection{IS-MDP: Equi-Invariant Property}
We first present a useful symmetrical property existing in IS-MDP, referred to as
{\em Equi-Invariance} (EI), which will be formally stated next.

\begin{comment}
exploiting the fact that the state $s_k \in \cS_k$ in each $k$ phase is a set so that the ordering of elements does not affect the behavior of IS-MDP, which in turn makes it possible to reduce state and/or action spaces.
\end{comment}

% Our description is applied for each phase $k \in \{0, \cdots, K-1\}.$
Recall the definition $s = (\bx,\bi) \in \cS_{k}$ in IS-MDP.
 The tuples $\bx$ and $\bi$  are actually sets since the orders of the items in $\bx$ and $\bi$ are not important in IS-MDP.
 Therefore, we can define a permutation $\sigma_{s}:=(\sigma_{x}, \sigma_{i}) \in \bS_{k} \times \bS_{N-k}$ for the state $s$ as
 \begin{align} \label{eq:sigma_s}
  \sigma_{s}(s) := (\sigma_{x}(\bx), \sigma_{i}(\bi)).
  \end{align}
  % where $\sigma_{x}$ and  $\sigma_{y}$ permute the elements in $\bx$ and $\by$ respectively.
  % where $\sigma_{x}(\bx):=(x_{\sigma_{x}(1)}, \cdots, x_{\sigma_{x}(k)})$ and  $\sigma_{i}(\bi):=(i_{\sigma_{i}(1)}, \cdots, i_{\sigma_{i}(N-k)})$.
  Both $s$ and $\sigma_{s}(s)$ are \textit{equivalent} from the perspective of the optimal
  policy $\pi^{\star}$ 
  % which implies that if the orders of items are changed by $\sigma_{s}$, the optimal agent is able to select the same item with the corresponding order i.e.,
\begin{align} \label{eq:Q(s,a)Invariant}
  \forall s \in \cS, \, \forall a \in \cA, \quad  Q^{\star}(s,a)\equiv Q^{\star}(\sigma_{s}(s),\sigma_{i}(a)).
\end{align}
The above statement can be directly dervied from the result of \cite{zinkevich2001symmetry}.

Recall that we have more attention to $Q^{\star}(s):\cS \rightarrow \Real^{\vert \cA(s)\vert}$ rather than $Q^{\star}(s,a)$ for the computational issue.
In IS-MDP, for a state $s= (\bx,\bi) \in \cS_{k}=\cX^{k} \otimes \cI^{N-k}$,
\begin{equation} \label{eq:Q(s)optimal}
Q^{\star}(\bx,\bi) := (q_{k+1}, \cdots, q_{N}) \in \Real^{N-k} \times \Real^{C} 
\end{equation}
where $q_{n}\in \Real^{C}$ represents $C$-dimensional vector of Q-values after selecting an item $i_{n}$ with $C$ possible commands.
% We denote $\sigma_{i}$ to $Q^{\star}(s)$ as
%  $$\sigma_{i}(Q^{\star}(\bx,\bi)):=(q_{\sigma_{i}(1)}, \cdots, q_{\sigma_{i}(N-k)}). $$
The below proposition is rewritten form of \eqref{eq:Q(s,a)Invariant} for $Q^{\star}(s)$.
\begin{prop} [Equi-Invariance in IS-MDP]
  \label{prop:ei_optimal}
  In IS-MDP, the optimal Q-function $Q^\star(\bx,\bi)$ is invariant to the order of $\bx$ as well as equivariant to the order of $\bi$, i.e., for any permutation $\sigma=(\sigma_x, \sigma_i)$,
\begin{align} \label{eq:equi-inv property}
  Q^\star(\sigma_{s}(s)) = Q^{\star}(\sigma_{x}(\bx), \sigma_{i}(\bi)) = \sigma_{i}(Q^{\star}(s)).
\end{align}
\end{prop}
We called this symmetry as permutational \textit{Equi-Invariance} (EI).
Since EI includes the concepts of both equivariance and invariance, EI can be regarded as an extended concept of permutation equivariance and invariance.



%   $ \\\\ $

% $$ Q^{\star}(s) := [Q^{\star}(s,a)]_{a \in \cA(s)} \in \Real^{N-k} \otimes \Real^{C} $$
% We define $Q^{\star}(s)$ as below with the definition of $\cA(s)$ in \eqref{eq:action space}.
%   can be regarded as the \textit{equivalent} states.
% %  the concatenation of individually applying permutation
% % \footnote{We abuse the same notation $\sigma$ for any dimensional vectors, unless confusion arises.}
% % \begin{align} \label{eq:sigma_s}
% % \sigma(s) := (\sigma_{x}(\bx), \sigma_{i}(\bi)).
% % \end{align}

% $\sigma_{s}:=(\sigma_x, \sigma_i)$

% \begin{comment}
% We first define a permutation $\sigma$ of a state $s_k = (\bx,\by)$, where $\bx = \{x_1,\ldots,x_k\}$ and $\by = \{y_1,\ldots,y_{N-k}\}$ are both sets, as
% \begin{align} \label{eq:sigma_s}
% \sigma(s_k) := (\sigma_k(\bx), \sigma_{N-k}(\by)),
% \end{align}
% for any permutations $\sigma_k$ and $\sigma_{N-k}$ of $k$ and $N-k$ elements, respectively, i.e.,
% \begin{align*}
% \sigma_k(\bx) = \{ x_{\sigma_k(1)}, \ldots, x_{\sigma_k(k)}\}, ~~\text{and}~~ \sigma_{N-k}(\by) = \{ y_{\sigma_{N-k}(1)}, \ldots, y_{\sigma_{N-k}(N-k)} \}.
% \end{align*}
% \end{comment}
% Then, it is easy to see that the reward and transition functions in IS-MDP are invariant to the permutation $\sigma$: for $s_k \in \cS_k$ and $a_k \in \cA_k(s_k)$,
% \begin{equation} \label{eq:tranGREEDYSEL}
%   \begin{split}
%  \cP(s_{k+1},  r_{k} \mid s_k,a_k) & = \cP(s_{k+1},r_{k} \mid \sigma(s_k),\sigma_{y}(a_k)).
% \end{split}
% \end{equation}
% % $$
% % Q(s_k) =
% % \begin{pmatrix}
% % Q(s_{k}, (y_{1}, c)) & \cdots  & \\
% % Q(s_{k}, (y_{2}, c))  & \cdots &  \\
% % \ddots & \vdots
% % \end{pmatrix}
% % $$
% % As mentioned in Section~\ref{sec:greedy-mdp}, the action space $\cA_k(s_k)$ is defined as
% % $$\cA_k(s_k)=[[(i,c)]_{c \in \cC}]_{i \in \by_{k}}. $$
% Proposition~\ref{prop:ei_optimal} states the similar but slightly different permutation property for the case of Q-function $Q(s_{k})$ which can be derived from transition property in \eqref{eq:equi-inv property}.

% % DP has the following so-called Equi-Invariant property (simply EI property) to the permutation of unselected and selected elements, as stated next.
% %e.g., $Q(s_k) = [Q(s_k,(i,c))]_{i \in \by, c \in \cC}$
% \begin{prop} [Equi-Invariance in IS-MDP]
%   \label{prop:ei_optimal}
%   In IS-MDP, for any phase $ 0 \leq k < K$ and for any given state $s_k = (\bx_k,\by_k),$ the optimal action value function $Q^\star(s_k)$ is invariant to $\sigma_{x}(\bx_k)$, and equivariant to $\sigma_{y}(\by_k)$, i.e., for any permutation $\sigma=(\sigma_x, \sigma_y)$,
% \begin{align} \label{eq:equi-inv property}
%   Q^\star(\sigma(s_k)) = Q^{\star}(\sigma_{x}(\bx_k), \sigma_{y}(\by_k)) = \sigma_{y}(Q^{\star}(s_{k})).
% \end{align}
% \end{prop}
% The result of proposition is just a paraphrased version of the following fact that $Q^{\star}(s_k,a_k) = Q^{\star}( \sigma(s_k), a_k)$ which can be easily induced from \eqref{eq:tranGREEDYSEL}.
% \note{This implies that the orders of the items in $\bx_{k}$ or $\by_{k}$ do not affect the optimal action values of the state $s_{k} =(\bx_{k}, \by_{k}) $.}
% However, the expression in \eqref{eq:equi-inv property} has different form since the $j$th row in $Q^{\star}(s_{k})$ represents the action values of $\{(y_{j}, c)\}_{c \in \cC}$.
% \note{
% Therefore, if the orders of the remaining items in $\by_{k}$ are permuted by $\sigma_{y}$, the rows in the matrix $Q^{\star}(s_{k})$ would be also permuted accordingly.
% By the way, the order in $\bx$ does not have any affect to the orders of q-values in $Q^{\star}(s_k)$.
% To sum up, $Q^{\star}(s_{k})$ or $Q^{\star}(\bx_{k}, \by_{k})$ is permutation invariant to $\bx_{k}$
% while it is permutation equivariant to $\by_{k}$.
% }
% This is the reason why we call this property as equi-invariance (EI).
% In Section \ref{sec:greedy-select-dqn}, we design a Q-network architecture which exploits EI of Q-networks.

% $ \\\\ $
\iffalse
\subsection{Old:IS-MDP: Equi-Invariant Property}
We first present a useful symmetrical property existing in IS-MDP, referred to as
{\em Equi-Invariance} (EI), which will be formally stated next.

\begin{comment}
exploiting the fact that the state $s_k \in \cS_k$ in each $k$ phase is a set, so that the ordering of elements does not affect the behavior of IS-MDP, which in turn makes it possible to reduce state and/or action spaces.
\end{comment}

Our description is applied for each phase $k \in \{0, \cdots, K-1\}.$
Recall that we consider a state $s_k = (\bx_k,\by_k)$, where $\bx_k = \{x_1,\ldots,x_k\}$ and $\by_k = \{y_1,\ldots,y_{N-k}\}$ are the sets, corresponding to the selected (item,command) pairs, and the unselected items, respectively. Then, we define a permutation $\sigma=(\sigma_x, \sigma_y)$ of a state $s_k$ where  $\sigma_x \in \bS_{k}$ and $ \sigma_y \in \bS_{N-k}$ implies the permutations for $\bx_k$ and $\by_k$ as:
%  the concatenation of individually applying permutation
% \footnote{We abuse the same notation $\sigma$ for any dimensional vectors, unless confusion arises.}
\begin{align} \label{eq:sigma_s}
\sigma(s_k) := (\sigma_{x}(\bx_k), \sigma_{y}(\by_k)).
\end{align}

\begin{comment}
We first define a permutation $\sigma$ of a state $s_k = (\bx,\by)$, where $\bx = \{x_1,\ldots,x_k\}$ and $\by = \{y_1,\ldots,y_{N-k}\}$ are both sets, as
\begin{align} \label{eq:sigma_s}
\sigma(s_k) := (\sigma_k(\bx), \sigma_{N-k}(\by)),
\end{align}
for any permutations $\sigma_k$ and $\sigma_{N-k}$ of $k$ and $N-k$ elements, respectively, i.e.,
\begin{align*}
\sigma_k(\bx) = \{ x_{\sigma_k(1)}, \ldots, x_{\sigma_k(k)}\}, ~~\text{and}~~ \sigma_{N-k}(\by) = \{ y_{\sigma_{N-k}(1)}, \ldots, y_{\sigma_{N-k}(N-k)} \}.
\end{align*}
\end{comment}
Then, it is easy to see that the reward and transition functions in IS-MDP are invariant to the permutation $\sigma$: for $s_k \in \cS_k$ and $a_k \in \cA_k(s_k)$,
\begin{equation} \label{eq:tranGREEDYSEL}
  \begin{split}
  \cR(s_k,a_k) & = \cR( \sigma(s_k), \sigma_{y}(a_k)), \\
 \cP(s_{k+1},  r_{k} \mid s_k,a_k) & = \cP(s_{k+1},r_{k} \mid \sigma(s_k),\sigma_{y}(a_k)).
\end{split}
\end{equation}
Let $Q^{\star}(s_k) := [Q^{\star}(s_k,a_k)]_{a_k \in \cA_k(s_k)} \in \Real^{N-k} \otimes \Real^{\vert \cC \vert}$ to denote all posible action values for $s_k$. Recall the definition of $\cA_k(s_k)$ in Section~\ref{sec:greedy-mdp},
$$\cA_k(s_k) = \{ (i,c) \mid i \in \by_{k}, c \in \cC \},$$ which implies that the rows are related to the selected item $i$ and the columns are related to the command  $c$. Representing Q-function like this way is frequently used in DQN since it reduces the computation cost by computing all q-values at once.


% $$
% Q(s_k) =
% \begin{pmatrix}
% Q(s_{k}, (y_{1}, c)) & \cdots  & \\
% Q(s_{k}, (y_{2}, c))  & \cdots &  \\
% \ddots & \vdots
% \end{pmatrix}
% $$
% As mentioned in Section~\ref{sec:greedy-mdp}, the action space $\cA_k(s_k)$ is defined as
% $$\cA_k(s_k)=[[(i,c)]_{c \in \cC}]_{i \in \by_{k}}. $$
Proposition~\ref{prop:ei_optimal} states the similar but slightly different permutation property for the case of Q-function $Q(s_{k})$ which can be derived from transition property in \eqref{eq:equi-inv property}.

% DP has the following so-called Equi-Invariant property (simply EI property) to the permutation of unselected and selected elements, as stated next.
%e.g., $Q(s_k) = [Q(s_k,(i,c))]_{i \in \by, c \in \cC}$
\begin{prop} [Equi-Invariance in IS-MDP]
  \label{prop:ei_optimal}
  In IS-MDP, for any phase $ 0 \leq k < K$ and for any given state $s_k = (\bx_k,\by_k),$ the optimal action value function $Q^\star(s_k)$ is invariant to $\sigma_{x}(\bx_k)$, and equivariant to $\sigma_{y}(\by_k)$, i.e., for any permutation $\sigma=(\sigma_x, \sigma_y)$,
\begin{align} \label{eq:equi-inv property}
  Q^\star(\sigma(s_k)) = Q^{\star}(\sigma_{x}(\bx_k), \sigma_{y}(\by_k)) = \sigma_{y}(Q^{\star}(s_{k})).
\end{align}
\end{prop}
The result of proposition is just a paraphrased version of the following fact that $Q^{\star}(s_k,a_k) = Q^{\star}( \sigma(s_k), a_k)$ which can be easily induced from \eqref{eq:tranGREEDYSEL}.
This implies that the orders of the items in $\bx_{k}$ or $\by_{k}$ do not affect the optimal action values of the state $s_{k} =(\bx_{k}, \by_{k}) $.
However, the expression in \eqref{eq:equi-inv property} has different form since the $j$th row in $Q^{\star}(s_{k})$ represents the action values of $\{(y_{j}, c)\}_{c \in \cC}$.
Therefore, if the orders of the remaining items in $\by_{k}$ are permuted by $\sigma_{y}$, the rows in the matrix $Q^{\star}(s_{k})$ would be also permuted accordingly.
By the way, the order in $\bx$ does not have any affect to the orders of q-values in $Q^{\star}(s_k)$.
To sum up, $Q^{\star}(s_{k})$ or $Q^{\star}(\bx_{k}, \by_{k})$ is permutation invariant to $\bx_{k}$
while it is permutation equivariant to $\by_{k}$.
This is the reason why we call this property as equi-invariance (EI).
In Section \ref{sec:greedy-select-dqn}, we design a Q-network architecture which exploits EI of Q-networks.
\fi
% However, due to the definition of $Q^{\star}(s_k)$, it does not need to consider the orders of the unselected items, but the $i$th row
% It is pretty obvious since the order of the selected items
% The equation \eqref{eq:equi-inv property} represents the above fact with the different form since $Q^{\star}(s_{k})$ is defined by the form of matrix.
% In IS-MDP, when the agent selects $k$th item, the order of the  selected $(k-1)^{th}$ items is not important.
% For example,
% Therefore, the action-values are \textit{invariant} to orders of $x_{k}$s. In contrast to, the order of the contexts of $y$s directly affects the corresponding action-values. For example, the action values of choosing $y_{1}$ among $\{2, 3\}$ and choosing $y_{2}$ among $\{3,2\}$ have the same action-value.
% It
% The EI property of our IS-MDP plays a critical role in reducing the state space for IS-MDP, i.e., ignore the redundant states through permutations.

\begin{comment}
\begin{prop} [Equi-Invariance in IS-MDP]
  \label{prop:ei_optimal}
  In IS-MDP, for any phase $ 0 \leq k \leq K$ and for any given state $s_k = (\bx_k,\by_k),$ the optimal action value function $Q^\star(s_k)$ is invariant to $\sigma(\bx_k)$, and equivariant to $\sigma(\by_k)$, i.e., for any permutation $\sigma$,
\begin{align} \label{eq:equi-inv property}
  Q^\star(\sigma(s_k)) = Q^{\star}(\sigma_{k}(\bx), \sigma_{N-k}(\by)) = \sigma_{N-k} (Q^{\star}(s_{k})). \end{align}
\end{prop}
The EI property of our IS-MDP plays a critical role in reducing the state space for IS-MDP, i.e., ignore the redundant states through permutations.
\end{comment}


%\note{interpretation as a symmetry. }

\begin{comment}
In this subsection, we induce a symmetry called EI property in the optimal action-value function  $\tQ^{\star}(\ts, \ta)$.
We found permutation invariant property of the transitions in IS-MDP \eqref{eq:tranGREEDYSEL}.
Recall that state $\ts_{k}:=(\tbx, \tby)$ can be represented as a tuple of sets where $\tbx:=\{x_{1}, \cdots, x_{k}\}$ and $\tby:=\{y_{1}, \cdots, y_{N-k}\}$ for $k=0, \cdots, K-1$.
The order of the items in $\tbx$ or  in $\tby$ does not affect to the state $\ts_{k} = (\tbx, \tby)$, i.e.,
for any permutations of $k$ and $N-k$, $\sigma_{k}\in \bS_{k}$ and $\sigma_{N-k } \in \bS_{N-k}$ respectively, we define $$\sigma_{k}(\bx):=\{x_{\sigma_{k}(1)}, \cdots, x_{\sigma_{k}(k)}\}, \qquad \sigma_{N-k}(\by):=\{y_{\sigma_{N-k}(1)}, \cdots, y_{\sigma_{N-k}(N-k)}\}. $$
Furthemore, we set
$\sigma(\ts_{k})$ as
\begin{gather} \label{eq:sigma_s}
   \sigma(\ts_{k}) := ( \sigma_{k}(\tbx), \sigma_{N-k}(\tby)).
\end{gather}
% \begin{align} \label{eq:sigma_s}

% \end{align}
The following state-action pairs $(s_{k}, a_{k})$ and $(\sigma_{s_{k}}(s_{k}), \sigma_{N-k}(\tby))$ shares the same reward and transition probability function, i.e.,
\begin{align} \label{eq:tranGREEDYSEL}
 & \cR(s_{k}, a_{k}) = \cR(\sigma(s_{k}),  \sigma_{N-k}(a_{k})), \quad
\cP(s_{k} ', \tr \mid s_{k}, a_{k})) = \cP(s_{k} ', \tr \mid \sigma(s_{k}),  \sigma_{N-k}(a_{k}))).
\end{align}

Now, we can derive the EI property of the optimal action value function $Q^{\star}(s_{k})$ from the symmetry in \eqref{eq:tranGREEDYSEL}. For convenient connected to our DQN design in Section \ref{sec:greedy-select-dqn}, we define the optimal action value functions as \begin{align} \label{eq:Qvalueopt}
[\tQ^{\star}_{k}(\ts_{k})]_{i\in \by, c \in \cC}:= \tQ^{\star}_{k}(\ts_{k}, (i, c) ).
\end{align}
\begin{prop} [Equi-Invariant Property]
  \label{prop:ei_optimal}
If we follow the above definition of $Q^{\star}_{k}(\ts_{k})$,
for all $\sigma_{k}$ and $\sigma_{N-k }$,
\begin{equation} \label{eq:equi-inv property}
  \tQ_{k}^{\star}(\sigma_{k}(\tbx),  \sigma_{N-k}(\tby)) =  \sigma_{N-k } (\tQ_{k}^{\star}(\ts_{k})).
\end{equation}
We will say that  function $F$ has  \textit{permutation Equi-Invariant property} to the $\tby$ and $\tbx$ (EI property) if $F$ satisfies \eqref{eq:equi-inv property}.
\end{prop}
EI property is very powerful property in reducing number of state-action pairs by ignoring the permutations of the orders of the items.
In the next section, we will present our DQN algorithm and our neural network architecture with the EI property to exploit this property.
The general relationship of symmetries between the transition functions and the optimal value functions were studied by
\citet{zinkevich2001symmetry}.
Our proposition with EI property in the optimal q-functions can be regarded as a special case of their works.
\end{comment}

% \vspace{-0.05cm}
\subsection{Iterative Select Q-learning (ISQ)}
\label{sec:greedy-select-dqn}
% \vspace{-0.05cm}
\paragraph{Cascaded Q-networks}
Recall \eqref{eq:Q(s)optimal} that the optimal Q-functions $Q^{\star}(s)$ have different input and output  state dimensions depends on phase $k$.
Introducing IS-MDP to DQN motivates us to build $K$ cascaded Q-networks per each phase $k$, as illustrated in Figure~\ref{fig:Perphase_networks}.
 $$Q_k(s; \omega_{k}): \set{S_k} \mapsto \real^{N-k} \otimes \real^{C}.$$
 $Q_k(\cdot \, ; \omega_{k})$ represents the Q-network for phase $k$ while $\omega_{k}$ and $\omega_{k}'$ represent the main and the  target parameters. 
 Each $Q_{k}(s \, ; \omega_{k})$ selects $(k+1)$th item with a command while considering the (information, command) of the previous selected items $\bx$ and the information of the remaine items $\bi$. 
 Denote $\bomega:=(\omega_{0},\cdots,\omega_{K-1}) $ and $\bomega':=(\omega'_{0}, \cdots,\omega'_{K-1})$ are collections of the main and the target weight parameters for all phases.
% Accordingly, the loss functions $l_{k}$ for experience $(s,a,r,s')$ are defined  differently depends on phase $k$ of $s$ as below. 
%  (i) for $0 \leq k < K-1,$
%  \begin{multline} \label{eq:loss_k}
%    l_{k}(\omega_{k}, \omega_{k+1}'):=
%    \left (\tQ_{k}(s,a) - \max_{a' \in \cA(s)}
%        \tQ_{k+1}(\ts', a') \right)^{2},
%    \end{multline}
%    % \item for $k=K-1,$
%  (ii) $k=K-1,$
%    \begin{multline} \label{eq:loss_K-1}
%     l_{k}(\omega_{k}, \omega_{k+1}'):=
%     \left (\tQ_{k}(s,a) - (r+ \gamma \max_{a'\in \cA(s)}
%         \tQ_{k+1}(\ts', a'))\right)^{2},
%    \end{multline}
% The above definition is a conversion of the loss function $L_{\omega}$ in \eqref{eq:loss_general} for general DQN.
% We differentiate the main Q-network $Q_{k}$ for current p-state $s_{k}$ from the target Q-network $Q_{k+1}$ for the next p-state $s_{k+1}$.
% The phase $k=K-1$ also can be handled  similarly. 
% We set the discount factor equals to $\gamma$ only at final phase $K-1$ and set $1$ in the remaining cases for $k<K-1$.
% This is not strictly necessary, but we guess this method would help the inter-sharing among the cascaded Q-networks   described in Section \ref{sec:Intersharing}.
% is updated using the transition experience $(\ts_{k}, \ta_{k}, \tr, \ts_{k+1})$ sampled from the $k^{th}$ replay buffer.
\begin{figure*}[ht]
  \centering
  % \includegraphics[width=0.9\linewidth]{figure/Perphase_networks}
  \includegraphics[width=.95\linewidth]{figure/net-structure}
  \caption{Simple example of weight shared Q-networks $Q_{k}(\cdot \, ; \theta_{k})$s when $K=3, N=4$.
In I-sharing in Section~\ref{sec:EINET}, the weights with the same color in the same layer layer in each Q-network $Q_{k}$ are tied together.
In only I-sharing, the weight parameter vectors $\theta_{l} $ and $\theta_{m}$ can be different.
In contrast, in U-sharing,
all the same colored weights even in distinct Q-networks also share the weight parameters, i.e.,
$\theta_{0} = \cdots = \theta_{3}$ in U-sharing.}
  \label{fig:Perphase_networks}
\end{figure*}

It is true that IS-DQN requires the $K$ distinct Q-networks and the width of each Q-network grows as the number of the item $N$ increases.
This fact can be problematic in scalability when $N$ or $K$ grows.
In the following sections, we propose a two-levels of parameter sharing: intra-parameter sharing and progressive-parameter sharing, which overcomes such weakness, which is one of our key contributions of this paper.
% 0216
% In Section \ref{sec:EINET}, we suggest a first level of parameter sharing for each $Q_{k}$ which called intra-sharing.
% In Section \ref{sec:Intersharing},  we suggest an second level of parameter-sharing between the distinct $Q_{k}$s for all $k = 0,1, \cdots, K-1$.

% as $K$ grows and requires large number of parameters when $N$ is large,
% which induces large computation cost, overfitting, and slow convergence.
% To handle both large $N$ and $K$, we present two parameter sharing methods:
% intra-parameter sharing (Section~\ref{sec:EINET}) and
% inter-parameter sharing (Section~\ref{sec:Intersharing}).

% \vspace{-0.2cm}
% \vspace{-0.05cm}


\iffalse
\subsubsection{Cascaded Q-networks}
Recall Section \ref{sec:greedy-select-dqn} that the optimal Q-functions $Q^{\star}(s_{k})$ have different input state dimensions and  output action-value dimensions since the dimensions of p-state $s_k = (\bx_{k}, \by_{k})$ and coupled action sets  $\set{A}_k(s_{k}) = \{ (i,c) \mid i \in \by_{k}, c \in \cC \} $ vary as $k$ changes.
Introducing IS-MDP to our problem makes the Q-function at phase $k$ endowed with different dimensions of input and output vectors for each phase $k,$ i.e., the phase-$k$ Q-function $Q_k: \set{S_k} \mapsto \real^{N-k} \otimes \real^{\vert \cC \vert}.$

This motivates us to build $K$ cascaded Q-networks $[\tQ(\ts_{k};\omega_k)]_{k=0}^{K-1}$, as illustrated in Figure~\ref{fig:Perphase_networks}.
With these cascaded Q-networks, there are $k$-phase loss functions $l_{k}(\omega_{k})$ for each phase $k$ for transition $(s_{k}, a_{k}, r_{k}, s_{k+1})$ are also defined:
% One difficulty to design a single network $\tQ(\ts;\omega)$ for IS-MDP is that both input and output dimensions of $\tQ(\ts_{k};\omega)$ are different for various values of $k$.
% Therefore, we propose to use $K$ separate neural networks $\tQ_{k}(\ts_{k} ; \omega_{k}), 0 \leq k < K$ for $K$ different dimensions of state $s_{k}$.
% Figure~\ref{fig:Perphase_networks} illustrates how these $K$ networks work.
% During selecting a $K$ combinated action $a=\{(n_{1},c_{1}), \cdots, (n_{K}, c_{K}) \}$,
% for each phase $k$, each $Q_{k}$ selects the $k^{th}$ pair of $\{$item, command$\}$ only and transfers the next intermediate state $s_{k+1}$ to the next Q-network $Q_{k+1}$.
% This process goes until the last $Q_{K-1}$ selects its $(K-1)^{th}$ pair.
% The divided $K$ phase are saved in the replay buffers.
% The loss function $L_{k}(\omega_{k})$ is also  defined with the consideration of the fact as follows:
%
%% previous equation 12/31
% \begin{compactenum}[(i)]
% \item for $0 \leq k \leq K-1,$
% \begin{multline} \label{eq:loss_k}
% l_{k}(\ts_{k}, \ta_{k}, 0, \ts_{k+1}  ; \omega_{k}):= \cr
% \left (\tQ_{k}(\ts_{k},\ta_{k};\omega_{k}) - (0 + 1 \cdot \max_{\ta_{k+1} \in \tcA_{k+1}(\ts_{k+1})}
%     \tQ_{k+1}(\ts_{k+1},\ta_{k+1};\omega_{k+1} ')) \right)^{2},
% \end{multline}
% \item for $k=K-1,$
% \begin{multline} \label{eq:loss_K-1}
% l_{K-1}(\ts_{K-1}, \ta_{K-1}, r, s'  ; \omega_{K-1}):= \cr
% \left (\tQ_{K-1}(\ts_{K-1},\ta_{K-1};\omega_{K-1}) - (\tr  + \gamma \max_{\ta ' \in \tcA_{0}(\ts')}
%     \tQ_{0}(\ts ',\ta ';\omega_{0} ')) \right)^{2}.
% \end{multline}
% \end{compactenum}
  % \begin{compactenum}[(i)]
  %   \item for $0 \leq k < K-1,$
  (i) for $0 \leq k < K-1,$
  \begin{multline} \label{eq:loss_k}
    l_{k}(s_{k}, a_{k}, r_{k}, s_{k+1}):= \cr
    \left (\tQ_{k}(\ts_{k},\ta_{k}) - \max_{\ta_{k+1} \in \tcA_{k+1}}
        \tQ_{k+1}(\ts_{k+1},\ta_{k+1}) \right)^{2},
    \end{multline}
    % \item for $k=K-1,$
  (ii) $k=K-1,$
    \begin{multline} \label{eq:loss_K-1}
    l_{k}(s_{k}, a_{k}, r_{k}, s_{k+1}):= \cr
    \left (\tQ_{k}(\ts_{k},\ta_{k}) - (\tr  + \gamma \max_{\ta ' \in \tcA_{0}}
        \tQ_{0}(\ts ',\ta ')) \right)^{2}.
    \end{multline}
    % \end{compactenum}

% \begin{align*}
%    k <K-1: \quad & L_{k}(\ts_{k}, \ta_{k}, 0, \ts_{k+1}  ; \omega_{k}):= (\tQ_{k}(\ts_{k},\ta_{k};\omega_{k}) - (0 +  \max_{\ta_{k+1} \in \tcA(\ts)}
%     \tQ_{k+1}(\ts_{k+1},\ta_{k+1};\omega_{k+1} ')))^{2},\\
%     k = K-1: \quad & L_{K-1}(\ts_{K-1}, \ta_{K-1}, r, s'  ; \omega_{K-1}):= (\tQ_{K-1}(\ts,\ta;\omega) - (\tr  + \gamma \max_{\ta ' \in \tcA(\ts)}
%     \tQ_{0}(\ts ',\ta ';\omega_{0} ')))^{2}.
% \end{align*}
The above definition is a conversion of the loss function $L_{\omega}$ in \eqref{eq:loss_general} for general DQN.
We differentiate the main Q-network $Q_{k}$ for current p-state $s_{k}$ from the target Q-network $Q_{k+1}$ for the next p-state $s_{k+1}$.
% The phase $k=K-1$ also can be handled  similarly.
We set the discount factor equals to $\gamma$ only at final phase $K-1$ and set $1$ in the remaining cases for $k<K-1$.
This is not strictly necessary, but we guess this method would help the inter-sharing among the cascaded Q-networks   described in Section \ref{sec:Intersharing}.
% is updated using the transition experience $(\ts_{k}, \ta_{k}, \tr, \ts_{k+1})$ sampled from the $k^{th}$ replay buffer.

\begin{figure*}[ht]
  \centering
  % \includegraphics[width=0.9\linewidth]{figure/Perphase_networks}
  \includegraphics[width=.95\linewidth]{figure/net-structure}
  \caption{Simple example of per-phase Q-networks $Q_{k}$s and the loss function $l_{k}$s when $K=3, N=4$.
% There are $K$ different simplified per-phase Q-networks.
 The loss function $l_{k}$ is defined between p-state $s_{k}$ and $s_{k+1}$ since every transition from $\cS_{k} \rightarrow \cS_{k+1}$.
 In I-sharing in Section~\ref{sec:EINET}, the weights with the same color per each Q-network $Q_{k}$ have the same values. If U-sharing in Section~\ref{sec:Intersharing}, all the same colored weights even in different Q-networks also share the weight value with some normalizings.}
  \label{fig:Perphase_networks}
\end{figure*}

It is true that IS-DQN requires $K$ distinct Q-networks and the size of each Q-network grows as the number of the item $N$ increases.
This fact can be problematic in scalability when $N$ or $K$ is large.
In the following sections, we propose a novel two-levels of parameter sharing:intra-parameter sharing and progressive-parameter sharing, which overcomes such weakness, which is one of our key contributions of this paper.
\fi
% 0216
% In Section \ref{sec:EINET}, we suggest a first level of parameter sharing for each $Q_{k}$ which called intra-sharing.
% In Section \ref{sec:Intersharing},  we suggest an second level of parameter-sharing between the distinct $Q_{k}$s for all $k = 0,1, \cdots, K-1$.

% as $K$ grows and requires large number of parameters when $N$ is large,
% which induces large computation cost, overfitting, and slow convergence.
% To handle both large $N$ and $K$, we present two parameter sharing methods:
% intra-parameter sharing (Section~\ref{sec:EINET}) and
% inter-parameter sharing (Section~\ref{sec:Intersharing}).

% \vspace{-0.2cm}
% \vspace{-0.05cm}


\paragraph{Intra-Parameter Sharing}
\label{sec:EINET}
%% previous figure
% \begin{wrapfigure}[11]{R}{.55\textwidth}
%   \vspace{-12pt}
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \begin{minipage}{.8\textwidth}
%         \includegraphics[width=\linewidth]{figure/layer-a}
%       \end{minipage}
%       \caption{Layer $\phi_A$}
%       \label{fig:layer-a}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \begin{minipage}{.8\textwidth}
%         \includegraphics[width=\linewidth]{figure/layer-b}
%       \end{minipage}
%       \caption{Layer $\phi_B$}
%       \label{fig:layer-b}
%     \end{subfigure}
%     \caption{Two layers for intra-parameter sharing. The parameters with the same color share the same value.} \vspace{-0.2cm}
%     \label{fig:eilayers}
%   \end{wrapfigure}
We first present \textit{intra-parameter sharing} (I-sharing) to handle a large $N$ in IS-MDP.
It is used for each cascaded Q-network $Q_k(s)$ are forced to satisfiy EI in \eqref{eq:Q(s)optimal} so the network can cognize the equivalent states correctly. i.e., for all phase $k$, 
$$ \sigma_{s}=(\sigma_{x}, \sigma_{i}) \in \bS_{k}\otimes \bS_{N-k}, \quad Q_{k}(\sigma_{s}(s))\equiv\sigma_{i}(Q_{k}(s)).  $$ 
% In other words, $Q_k$ with I-sharing correctly estimates the action values which are not depended by the orders of the already selected items in $\bx$ or the remained items in $\bi$.
From now on, we denote $Q_{k}(\cdot \, ; \theta_{k})$ to represent the I-shared Q-network for phase $k$ where $\theta_{k}$ is a weight parameter vector for phase $k$.
Other notations including $\btheta=(\theta_{1}, \cdots, \theta_{K}), \theta_{k}',$ and $\btheta'=(\theta_{1}', \cdots, \theta_{K}')$ are defined similarly.
We sometimes omit $\theta_{k}$ and abuse  $Q_{k}(\cdot)$ or $Q_{k}$ to represent the I-shared network for notational convenience. 
% The key feature in this parameter sharing is about proposing a new neural network architecture
% that exploits a mixture of invariance and equivariance, formalized in Proposition~\ref{prop:ei_optimal} or \eqref{eq:equi-inv property}.
% \note{HS: recall that the output $Q_k$ }


Layers that make up the I-shared Q-network $Q_{k}(\cdot \, ; \theta_{k})$
 are classified to two types of parameter-shared layers: $\phi_{k}$ and $\psi_{k}$.
Both types of layers satisfy special permutational properties to force $Q_{k}$ to satisfy EI in \eqref{eq:Q(s)optimal}.
 The layer $\phi_{k}$ can be stacking up multiple times ($D \geq 1$ times) while the anonther layer $\psi_{k}$ is only used as the last output layer in $Q_{k}$. i.e.,
 $$Q_{k}(s \, ; \theta_{k}):=\psi_{k} \circ \phi_{k}^{1} \circ \cdots \circ \phi_{k}^{D}(s)$$
 where $\phi_{k}^{1}, \cdots, \phi_{k}^{D}$ represent the $D$ stacked layers with the same type.
% The layers $\phi_{k}^{A}$ are stacking up multiple times and the layer $\phi_{k}^{B}$ is only used as the last output layer in $Q_{k}$.
The simple form of $Q_{k}$ is described in Figure \ref{fig:eilayers}.
Under the fact that the same colored weights in the same layer such as $\phi$ or $\psi$ are tied together,
the weight shared layers always preserve the orders of the items in $\bx$ or $\bi$.
\footnote{Our weight shared network design is a special case in \cite{ravanbakhsh2017equivariance}.}
i.e., for all 
 $ \sigma_{s} = (\sigma_{x}, \sigma_{i}) \in \bS_{k} \otimes \bS_{N-k}, $
\begin{equation*} \label{eq:layersymmetry}
  \begin{split}
   \phi_{k}(\sigma_{s}(\bx,\bi))\equiv & \sigma_{s}(  \phi_{k}(\bx,\bi)), \, \, \, \,
    \psi_{k}(\sigma_{s}(\bx,\bi)) \equiv \sigma_{i}(\psi_{k}(\bx,\bi)),
    \\
    & Q_{k}(\sigma_{s}(\bx,\bi)) \equiv \sigma_{i}(Q_{k}(\bx,\bi)).
  \end{split}
  \end{equation*}
% The layer $\phi_{k}^{A}$ can be regarded as  equivariant both $\bx, \by$ while $\phi_{k}^{B}$ is only equivariant to $\by$.
% In $Q_{k}$, all the layers except the output layer has structure of $\phi_{k}^{A}$ and the final output layer has structure of $\phi_{k}^{B}$ or  $Q_{k}:=\phi_{k}^{B} \circ \phi_{k}^{A} \circ \cdots \circ \phi_{k}^{A}.$
% It is easily induced from \eqref{eq:layersymmetry} that $Q_{k}$ satisfies EI.
% For presentational simplicity, in Figure \ref{fig:eilayers}, we simlify the case when $\bx_{k} \in \Real^{k}$, $\by_{k} \in \Real^{N-k}$ and $\vert \cC \vert =1$.
% We denote `ISQ-I' as an ISQ algorithm  with I-shared Q-networks.
 The complete description of our I-shared network will be given in Appendix \ref{sec:IntraSharing}.
 \footnote{Appendix and Codes are uploaded at \note{github links}.}

The intra-sharing is very efficient to handle when the number of item $N$ is large.
% It reduces a lot of weight parameter with the from the
It reduces the number of weights from $O(N^{2}K)$ for $\bomega$ to $O(K)$ for $\btheta$.
However, we still need to train $K$ distinct Q-networks which takes a long time as $K$ grows. 
% This is because that unlike to a general DQN, the  
% For example, for the Q-network $Q_{k}$ for phase $k$ to learn correctly, the other networks $Q_{k+1}, \cdots, Q_{K-1}$ for further phases should learn first.
In the following section, we share additional parameters among $K$ cascaded Q-networks by progressive-sharing to speed up the training of the cascaded Q-networks.

\iffalse
$ \\\\ $


The I-shared Q-network $Q_{k}$
 is composed  of two types of parameter-shared layers $\phi_{k}^{A}$ and  $\phi_{k}^{B}$ which both layers satisfy special permutational properties so $Q_{k}$ also satisfies EI.
The layers $\phi_{k}^{A}$ are stacking up multiple times and the layer $\phi_{k}^{B}$ is only used as the last output layer in $Q_{k}$.
The simple form of $Q_{k}$ is described in Figure \ref{fig:eilayers}.
Under the fact that the same colored weights in the same layer are tied together, the layer $\phi_{k}^{A}$ preserves the orders of both the selected items $\bx$ and  unselected items $\by$ while the layer $\phi_{k}^{B}$ preserves the order of the only selected items in $\by$. Therefore, $Q_{k}$ preserves the order of the items in $\by$ (permutation equivariant) and equally treats the selected items in $\bx$ (permutation invariant),
% To explain more specifically why $Q_{k}$ satisfies EI, firstly consider the relationship between the input nodes and output nodes in  $\phi_{k}^{A}$. For example, suppose that the order of the nodes $x_{1}, x_{2}$ is changed, the order of the output nodes $h_{1}^{x}, h_{2}^{x}$ would also be changed while other nodes maintain their values.
% However, even though $h_{1}^{x}, h_{2}^{x}$ are changed, the output q-values of layer $\phi_{k}^{B}$ does not depend from the change or implies that $Q_{k}$ is  permutation invariant to $\bx$ with the permutation $\sigma_{x}$.
% On the other hand, if the orders of $y_{1}, y_{2}$ change, both $h_{1}^{y}, h_{2}^{y}$ and $q_{1}, q_{2}$ follow this change which implies that $Q_{k}$ is permutation equivariant to $\by$ with the permutation $\sigma_{y}$,
i.e., $\forall \sigma = (\sigma_{x}, \sigma_{y}) \in \bS_{k} \otimes \bS_{N-k}, $
\note{proposition}
\begin{equation} \label{eq:layersymmetry}
  \begin{split}
   \phi_{k}^{A}(\sigma(\ts_{k}))= \sigma( & \phi_{k}^{A}(\ts_{k})), \, \, \, \,
    \phi_{k}^{B}(\sigma(\ts_{k})) = \sigma_{y}(\phi_{k}^{B}(\ts_{k})),
    \\
    & Q_{k}(\sigma(\ts_{k})) = \sigma_{y}(Q_{k}(\ts_{k})).
  \end{split}
  \end{equation}
The layer $\phi_{k}^{A}$ can be regarded as  equivariant both $\bx, \by$ while $\phi_{k}^{B}$ is only equivariant to $\by$.
In $Q_{k}$, all the layers except the output layer has structure of $\phi_{k}^{A}$ and the final output layer has structure of $\phi_{k}^{B}$ or  $Q_{k}:=\phi_{k}^{B} \circ \phi_{k}^{A} \circ \cdots \circ \phi_{k}^{A}.$
It is easily induced from \eqref{eq:layersymmetry} that $Q_{k}$ satisfies EI.
For presentational simplicity, in Figure \ref{fig:eilayers}, we simlify the case when $\bx_{k} \in \Real^{k}$, $\by_{k} \in \Real^{N-k}$ and $\vert \cC \vert =1$. The complete description of our intra-sharing will be given in Appendix \ref{sec:IntraSharing}.

The intra-sharing is very efficient to handle when the number of item $N$ is large.
% It reduces a lot of weight parameter with the from th
It only has the number of weights $O(K)$ compared to the same architecture neural network without sharing requires $O(N^{2}K)$ number of parameters.
However, it still have some problems when $K$ grows, since there would be $K$ cascaded Q-networks $Q_{k}(s_{k})$ exists.
In the following section, we shares additional parameters among $K$ cascaded Q-networks by inter-sharing method.

\fi

% Therefore, the $Q_{k}(\bx_{k}, \by_{k}): \Real^{k} \otimes \Real^{N-k} \rightarrow \Real^{N-k}$ where the $j$th element in the output vector implies the action values for $y_{j}$.


% \begin{align} \label{eq:layersymmetry}
%   \phi_{k}^{A}(\sigma(\ts_{k}))= \sigma(\phi_{k}^{A}(\ts_{k})), \quad
%     \phi_{k}^{B}(\sigma(\ts_{k})) = \sigma_{N-k}(\phi_{k}^{B}(\ts_{k})).
%    \end{align}

% As a result, $Q_{k}$ also always satisfies EI to $(\bx, \by)$ if we set $Q_{k}:=\phi_{k}^{B} \circ \phi_{k}^{A} \circ \cdots \circ \phi_{k}^{A}$.



% In this subsection, we explain the intra-parameter shared neural network architectures to approximate the optimal Q-functions $\tQ^{\star}_{k}(\ts_{k})$ with EI property in \ref{eq:equi-inv property}.
% The intra-parameter sharing makes to have the EI property to the networks.
% We first define two types of fully connected layers $\phi^{A}, \phi^{B}$ with the idea of {\em parameter sharing} and then combine multiple layers to make a deep neural network.

% and prove the local minimal parameter in the EINET is also the local minimal parameter in a same-architectured deep neural network without any parameter sharing.

%\smallskip \noindent {\bf Intra-Parameter Shared Layers.}
%\myparagraph{Intra-Parameter Shared Layers}


% We first present the simplest version of intra-parameter sharing method with single layers.
% We will present detailed explanation of intra-parameter sharing such as with multiple channels in the Appendix \ref{sec:multiplechannels}.


% \note{The following should be explained. Why we need two types of layers. What's the role of each layer? How are you connect them to make the final deep network? How many parameter reduction occurs?

% Reviewer's mind: They want to understand how well equivariance and invariance are realized in a mixed manner. They are ready to be surprised by our smartness, but we failed to surprise them.}


% We define two types of fully connected layers $\phi_{k}^{A}, \phi_{k}^{B}$ called intra-parameter shared layers.
% The basic architectures are elaborated in Figure~\ref{fig:eilayers}. The same colored weight parameters are tied together.
% The key intuition of intra-parameter sharing method is that shared the parameters so the layers have the EI property or do not be affected by the orders of the items such as $x_{j} \in \bx$ or $y_{j} \in \by$.
% There are two types of layer
% $\phi_{k}^{A}: \Real^{k} \otimes \Real^{N-k}  \mapsto \Real^{k} \otimes \Real^{N-k} $ and
% $\phi_{k}^{B}: \Real^{k} \otimes \Real^{N-k}  \mapsto \Real^{N-k} $ with the following property for any $\sigma_{k}(\bx)$,  $\sigma_{N-k}(\by)$, and $\sigma(s_{k})$ defined in \eqref{eq:sigma_s},
% %  \begin{align} \label{eq:layersymmetry}
% % \phi_{k}^{A}(\sigma(\ts_{k}))= \sigma(\phi_{k}^{A}(\ts_{k})), \hspace{0.15cm}
% %   \phi_{k}^{B}(\sigma(\ts_{k})) = \sigma_{N-k}(\phi_{k}^{B}(\ts_{k})), \hspace{0.15cm}  G(\ts_{k})= \phi_{k}^{B} \circ \phi_{k}^{A} \circ \cdots \circ \phi_{k}^{A}(\ts_{k}).
% %  \end{align}
%  The deep neural network $G(\ts_{k})$ is made up of composition of layers always satisfies EI property in \eqref{eq:equi-inv property}.
%  The detailed explanation of the layers are described in the appendix \ref{sec:IntraSharing}.
%  This intra-parameter sharing is very efficient to handle when $N$ is large since the parameter sharing ignores the orders of the items in $\bx$ or $\by$. However, it still have some problem when $K$ grows, since there would be large number of $Q_{k}(s_{k})$ exists.
%  In the following section, we shares additional parameters among $K$ cascaded Q-networks.


% \subsubsection{Progressive-Parameter Sharing}
\smallskip \noindent{ \bf Inter-Parameter Sharing.}
\label{sec:Intersharing}
% \note{What Reviewers want to know: (i) what is inter-parameter sharing? (ii) Why does it make sense? What intuition is working here? (iii) What's the expected weakness of this mehtod, and why is it expected to be insignificant? (iv) How many parameter reduction occurs? Thus, the total reduction from that without parameter sharing to that with intra- and inter-parameter sharing?}
In this subsection, we propose second-level inter parameter sharing methods among the I-shared Q-networks. 
We first introduce an observation before describing the detailed methods.
The observation is that each the I-shared Q-network $Q_{k}(\cdot \, ; \, \theta_{k})$ has a fixed number of the weight parameters regardless phase $k$. 
This fact is well described in Figure~\ref{fig:Perphase_networks} such as the numbers of different colors in $Q_{1}$ and $Q_{2}$ are the same.
From the observation, we additionaly share the weight parameters $\theta_{k}$ among the different Q-networks $Q_{k}$ as $\theta_{0} = \cdots = \theta_{K-1}$ which called \textit{unified-parameter sharing} (U-sharing).
From U-sharing, the number of the weight parameters is reduced greatly from $O(K)$ for $\btheta$ to $O(1)$ for $\theta_{0}= \cdots = \theta_{K-1}$.
This small number of weight paramaters helps the faster training of the Q-networks. 
The reason of our conjecture for U-sharing is that the criteria for item evaluation is similar at any phases since the order of the selected items does not affect the transition in S-MDP. 
Therefore, we can guess that there are some similarities among $Q_{k}$s which implies that the weight parameters $\theta_{k}$ may also have similar values.
However, an inherent problem still left from the reduced expressive power of $Q_{k}$s under the U-sharing.


To combine both advantages of I-sharing and U-sharing, we propose a different inter-parameter sharing method called \textit{progressive parameter-sharing} (P-sharing).
With P-sharing, we start with a single parameter vector (same as U-sharing) and then progressively increase the number of the parameter sets doubly until it reaches $K$ (same as I-sharing).
The Q-networks with nearby phases tends to share the same parameter set longer since we believe that $Q_{k_{1}}$ and $Q_{k_{2}}$ would have a similar role when $k_{1}$ and $k_{2}$ are nearby.
The detail is visualized in Figure~\ref{fig:Progressive_learning}.
In the early stage of the learning where the networks are not stable, the Q-networks are trained sample-efficiently as they exploit the advantages of U-sharing.
On the other hand, as the training progresses gradually, the Q-networks are able to be trained more elaborately by increasing the number of the parameter sets.
In P-sharing, the number of the total weight parameters increases from $O(1)$ to $O(K)$ during the training.

\begin{figure}[ht]
  \centering
  \includegraphics[width=.99\linewidth]{figure/Progressive_learning.pdf}
  \caption{Simple
   scenario for progressive-sharing when $K=4$. Initially, $\theta_{0} = \cdots = \theta_{3}$ which implies that whole $Q_{k}$s share their weights.  
  After a certain training step, $\theta_{0} = \theta_{1}$ and $\theta_{2} = \theta_{3}$. Finally, each Q-networks $Q_{k}$ has its own weight parameters $\theta_{k}$.  
  }
  \label{fig:Progressive_learning}
\end{figure}



%% Previous writing before 12/25
% There are two advantages of inter-sharing when $K$ grows.
% Firstly and most importantly, inter-sharing helps the cascaded Q-networks updates their q-values much more efficiently by sharing the parameters.
% Suppose that we use only intra-sharing method.
% When we update the cascaded Q-networks, only $Q_{K-1}$ updates its network with non-zero reward in the loss $l_{K-1}$ in \eqref{eq:loss_K-1}.
% Which means the other networks $Q_{0} \sim Q_{K-2}$ should wait until $Q_{K-1}$ learns some meaningful q-values.
% This updates cascades from $Q_{K-2}, \cdots, Q_{0}$ one by one.
% Therefore, it will takes some time until that these updates cascades to the last network $Q_{0}$.
% However, when we use inter-sharing, the other networks $Q_{k}$ for $0\leq k \leq K-2$ can be simultaneously updated when the agent just reduces the loss in $l_{K-1}$.
% The faster update of $Q_{0}$ would help  to update $Q_{K-1}$ again since $Q_{0}$ generates the target values in $l_{K-1}$ for given experience.
% Secondly, a small number of the parameters reduces the memory and computation cost during the gradient descent of the networks.
% For example, the numbers of parameters for IS-MDP(K,N) are $O(N^{2}K), O(K)$, $O(1)$ as we do not use any parameter sharing, using intra-sharing only, and inter-sharing method respectively.
% Furthermore, thanks to algorithms in tensorflow that increase the computation speed a lot when we use inter-sharing.
% The simulation results in Section \ref{sec:eval} strongly show both advantages of our inter-sharing method.

% In Figure~{\ref{fig:Perphase_networks}}, each $Q_{k}$ has some similar shapes and fixed number of parameters. For example, the yellow dot lines in $Q_{1}(s_{1})$ and $Q_{2}(s_{2})$ may have similar role to transfer the information (item, command) of the selected elements $x_{1}, x_{2}$.


% In inter-parameter sharing, the whole $Q_{k}$ shares the same weight value  with some normalization rule by specific $N,k$.
% By making this way, the number of the weight parameters in inter-parameter sharing methods  do not be affected by varying $K$.
% Furthermore, this inter-parameter sharing method facilitates  fast convergence of the training since each $Q_{k}$ shares their knowledge directly each others.

% In normal DQN case, the trained network would be useless when the size of $N$ differs.
% In our DQN algorithm with the similar manner to the intuition for inter-parameter sharing, the trained parameter of this network may be reused in another environment with different input dimension, such as $N=200$.




% In the previous EI-NN, $\ovt(x,y): R^{1} \rightarrow R^{1}$ are assigned between the $x_{i}$ and $h_{j}^{1,y}$.

% from $H_{\ovt} : R^{N+M} \rightarrow R^{M}$ to   $H_{\ovt} : R^{NK_{I}+MK_{E}} \rightarrow R^{M\times K_{O}} $ where $K_{I},K_{E}$, and $K_{O}$ is the number of the dimension for each elements $x$, $y$, and


% which handles the case when the input elements $x$ or $y$ have multiple features as well as the output of the policy $\pi$
% %  All nodes in the neural network can be regarded as $k$ dimensional vector rather than a simple $1$-dimensional value where $k$ is an arbitrary positive integer.
% The first layer $ \phi^{1}:R^{N+M} \rightarrow R^{N+M} $ of neural network $G_{g(\ovt)}$ can be extended to  $ \phi^{1}:R^{(N+M)\times K_{0}} \rightarrow R^{(N+M)\times K_{1}} $ where $K_{0},K_{1}$ is the number of the
% The shared weight parameters in $G_{g(\overline{\omega})}$ are also converted from $1$-dimensional value to proper dimensional matrix.
% %  such as $w_{x,y} ^{1,g}$
% For example, suppose that the invariant input elements $\bx_{i}$ has $k_{x}$ dimensional vector and the hidden node $\bh_{j}^{1,y}$ has $h_{y}$ dimensional vector.
% In this case, we can extend the $1$-dimensional weight parameter $w_{x,y} ^{1,g}$ to $h_{y} \times k_{x}$-dimensional matrix weight parameters $\bw_{x,y}^{1,g}$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> figure/abstract.tex <==
\begin{abstract}
We consider a problem of sequentially selecting $K$ items among $N$ items over time, which we model by so-called Select-MDP (S-MDP).  
Due to a sequence of combinatorial selections, thereby 
too large state and action spaces,  
learning a good policy is computationally intractable as $N$ grows.  
In this paper, we present a DQN-based deep reinforcement algorithm that finds a good policy
by adopting the following key ideas: We convert the original S-MDP into a equivalent one, called Iterative Select-MDP (IS-MDP). IS-MDP decomposes a joint action of selecting $K$ items simultaneously into $K$ iterative selections, resulting in reducing the number of actions per state at the expense of exponential increase in state space. 
This state space explosion is overcome by exploiting a special property of equi-invariance uniquely existing in IS-MDP and by developing significantly simplified $K$-cascaded deep Q-networks based on two levels of intra- and inter-parameter sharing thanks to equi-invariance in IS-MDP. We mathematically prove two theorems that guarantee the expressive power of our intra-shared neural network: `relative local optimality' and `universal approximity'. 
% of our scheme in the sense that the local optimum of our Q-network with intra-parameter sharing coincides with that of non-parameter shared Q-network with much larger expressive power. 
We evaluate the performance of our algorithm in two different environments of circle selection problem and predator-prey, where the agent should consider combinatorial effect of selection among numbers of items to get a high cumulative reward. 

% allows the agent to 
% iteratively chooses each item $K$


% tries to find an optimal policy  

% solves select-MDP
% with large $N$ by effectively integrating two techniques: 
% modifying the MDP through decomposition of the joint action space,
% and propose a parameter shared neural network to efficiently explore the large state space.
% We prove that the expressive power of the parameter shared neural network although this neural network reduces a lot of weight  parameters.  
% We demonstrate strong performance evaluation results on large-scale tasks in two types of environments which the agent must consider combinatorial effects of items to get the good performance.
  % and fast convergence compared to other methods.
\end{abstract}


% \note{HS:I think we should omit this. Usually, these large-scale SELECT-MDP is considered difficult to be solved via deep reinforcement learning because the agent needs to explore more state and action spaces as  the number of the elements increases.
% Furthermore, the deep neural networks are usually not suitable to handle the different scale of the elements during the training or test.}


==> figure/conclusion.tex <==
\section{Conclusion}
This paper has considered the problem of the sequential selection one element among large set. 
In this paper, we introduced select-MDP and a neural network architecture (EINET) with permutation equi-invariant property to approximate the Q-function.
EINET greatly reduced the number of parameters while preserving its expressive power.
We theoretically analyzed this by showing EINET still can achieve the local optimal weight parameters. 
We further suggested synchronous update algorithm by exploiting the EINET to learn the various  environments with different element size at one training. 
In the experiment of the Sequential Circle Selection, we demonstrated the robustness of DQN composed by EINET in large scale RL tasks
which could be affordable to learn 1000 circles while baseline DQNs could not afford only 50 circles.
Furthermore, we checked that we were able to train the weight parameters for the various environments with different size of elements by using the synchronous update algorithm.


==> figure/einn.tex <==
\section{Methods and Analysis}
\label{sec:Methods}

\begin{comment}
In this section, we explain how the proposed ideas in previous section
are utilized to construct our EINET and derive
a progressive algorithm to efficiently solve the select-MDP.
% In section~\ref{sec:greedy-select-dqn},
We first explain our greedy select-DQN algorithm with $K$ different Q-networks for greedy select-MDP with $K$ selections.
% In section~\ref{sec:EINET},
Then, we introduce our parameter shared neural network architecture for Q-networks, and provide mathematical analysis for optimality of the network.
% in section~\ref{sec:math-einet}.
Finally, some sharing techniques are proposed to make the algorithm more efficient.
% in section~\ref{sec:inter-intra}.
\end{comment}


\subsection{IS-MDP: Equi-Invariant Property}
We first present a useful symmetrical property existing in IS-MDP, referred to as  
{\em Equi-Invariance} (EI), which will be formally stated next. 

\begin{comment}
exploiting the fact that the state $s_k \in \cS_k$ in each $k$ phase is a set, so that the ordering of elements does not affect the behavior of IS-MDP, which in turn makes it possible to reduce state and/or action spaces. 
\end{comment}

Our description is applied for each phase $k \in \{0, \cdots, K-1\}.$ 
Recall that we consider a state $s_k = (\bx_k,\by_k)$, where $\bx_k = \{x_1,\ldots,x_k\}$ and $\by_k = \{y_1,\ldots,y_{N-k}\}$ are the sets, corresponding to the selected (item,command) pairs, and the unselected items, respectively. Then, we define a permutation $\sigma=(\sigma_x, \sigma_y)$ of a state $s_k$ where  $\sigma_x \in \bS_{k}$ and $ \sigma_y \in \bS_{N-k}$ implies the permutations for $\bx_k$ and $\by_k$ as: 
%  the concatenation of individually applying permutation
% \footnote{We abuse the same notation $\sigma$ for any dimensional vectors, unless confusion arises.} 
\begin{align} \label{eq:sigma_s}
\sigma(s_k) := (\sigma_{x}(\bx_k), \sigma_{y}(\by_k)).
\end{align}

\begin{comment}
We first define a permutation $\sigma$ of a state $s_k = (\bx,\by)$, where $\bx = \{x_1,\ldots,x_k\}$ and $\by = \{y_1,\ldots,y_{N-k}\}$ are both sets, as 
\begin{align} \label{eq:sigma_s}
\sigma(s_k) := (\sigma_k(\bx), \sigma_{N-k}(\by)),
\end{align}
for any permutations $\sigma_k$ and $\sigma_{N-k}$ of $k$ and $N-k$ elements, respectively, i.e., 
\begin{align*}
\sigma_k(\bx) = \{ x_{\sigma_k(1)}, \ldots, x_{\sigma_k(k)}\}, ~~\text{and}~~ \sigma_{N-k}(\by) = \{ y_{\sigma_{N-k}(1)}, \ldots, y_{\sigma_{N-k}(N-k)} \}.
\end{align*}
\end{comment}
Then, it is easy to see that the reward and transition functions in IS-MDP are invariant to the permutation $\sigma$: for $s_k \in \cS_k$ and $a_k \in \cA_k(s_k)$,
\begin{equation} \label{eq:tranGREEDYSEL}
  \begin{split}
  \cR(s_k,a_k) & = \cR( \sigma(s_k), \sigma_{y}(a_k)), \\
 \cP(s_{k+1},  r_{k} \mid s_k,a_k) & = \cP(s_{k+1},r_{k} \mid \sigma(s_k),\sigma_{y}(a_k)). 
\end{split}
\end{equation}
Let $Q^{\star}(s_k) := [Q^{\star}(s_k,a_k)]_{a_k \in \cA_k(s_k)} \in \Real^{N-k} \otimes \Real^{\vert \cC \vert}$ to denote all posible action values for $s_k$. Recall the definition of $\cA_k(s_k)$ in Section~\ref{sec:greedy-mdp}, 
$$\cA_k(s_k) = \{ (i,c) \mid i \in \by_{k}, c \in \cC \},$$ which implies that the rows are related to the selected item $i$ and the columns are related to the command  $c$. Representing Q-function like this way is frequently used in DQN since it reduces the computation cost by computing all q-values at once. 


% $$
% Q(s_k) = 
% \begin{pmatrix} 
% Q(s_{k}, (y_{1}, c)) & \cdots  & \\
% Q(s_{k}, (y_{2}, c))  & \cdots &  \\
% \ddots & \vdots 
% \end{pmatrix}
% $$
% As mentioned in Section~\ref{sec:greedy-mdp}, the action space $\cA_k(s_k)$ is defined as 
% $$\cA_k(s_k)=[[(i,c)]_{c \in \cC}]_{i \in \by_{k}}. $$
Proposition~\ref{prop:ei_optimal} states the similar but slightly different permutation property for the case of Q-function $Q(s_{k})$ which can be derived from transition property in \eqref{eq:equi-inv property}.

% DP has the following so-called Equi-Invariant property (simply EI property) to the permutation of unselected and selected elements, as stated next.
%e.g., $Q(s_k) = [Q(s_k,(i,c))]_{i \in \by, c \in \cC}$
\begin{prop} [Equi-Invariance in IS-MDP]
  \label{prop:ei_optimal}
  In IS-MDP, for any phase $ 0 \leq k < K$ and for any given state $s_k = (\bx_k,\by_k),$ the optimal action value function $Q^\star(s_k)$ is invariant to $\sigma_{x}(\bx_k)$, and equivariant to $\sigma_{y}(\by_k)$, i.e., for any permutation $\sigma=(\sigma_x, \sigma_y)$, 
\begin{align} \label{eq:equi-inv property}
  Q^\star(\sigma(s_k)) = Q^{\star}(\sigma_{x}(\bx_k), \sigma_{y}(\by_k)) = \sigma_{y}(Q^{\star}(s_{k})). 
\end{align}
\end{prop}
The result of proposition is just a paraphrased version of the following fact that $Q^{\star}(s_k,a_k) = Q^{\star}( \sigma(s_k), a_k)$ which can be easily induced from \eqref{eq:tranGREEDYSEL}.
This implies that the orders of the items in $\bx_{k}$ or $\by_{k}$ do not affect the optimal action values of the state $s_{k} =(\bx_{k}, \by_{k}) $.
However, the expression in \eqref{eq:equi-inv property} has different form since the $j$th row in $Q^{\star}(s_{k})$ represents the action values of $\{(y_{j}, c)\}_{c \in \cC}$.
Therefore, if the orders of the remaining items in $\by_{k}$ are permuted by $\sigma_{y}$, the rows in the matrix $Q^{\star}(s_{k})$ would be also permuted accordingly.
By the way, the order in $\bx$ does not have any affect to the orders of q-values in $Q^{\star}(s_k)$.
To sum up, $Q^{\star}(s_{k})$ or $Q^{\star}(\bx_{k}, \by_{k})$ is permutation invariant to $\bx_{k}$
while it is permutation equivariant to $\by_{k}$.
This is the reason why we call this property as equi-invariance (EI). 
In Section \ref{sec:greedy-select-dqn}, we design a Q-network architecture which exploits EI of Q-networks.  
% However, due to the definition of $Q^{\star}(s_k)$, it does not need to consider the orders of the unselected items, but the $i$th row 
% It is pretty obvious since the order of the selected items 
% The equation \eqref{eq:equi-inv property} represents the above fact with the different form since $Q^{\star}(s_{k})$ is defined by the form of matrix.
% In IS-MDP, when the agent selects $k$th item, the order of the  selected $(k-1)^{th}$ items is not important.
% For example, 
% Therefore, the action-values are \textit{invariant} to orders of $x_{k}$s. In contrast to, the order of the contexts of $y$s directly affects the corresponding action-values. For example, the action values of choosing $y_{1}$ among $\{2, 3\}$ and choosing $y_{2}$ among $\{3,2\}$ have the same action-value. 
% It 
% The EI property of our IS-MDP plays a critical role in reducing the state space for IS-MDP, i.e., ignore the redundant states through permutations.

\begin{comment}
\begin{prop} [Equi-Invariance in IS-MDP]
  \label{prop:ei_optimal}
  In IS-MDP, for any phase $ 0 \leq k \leq K$ and for any given state $s_k = (\bx_k,\by_k),$ the optimal action value function $Q^\star(s_k)$ is invariant to $\sigma(\bx_k)$, and equivariant to $\sigma(\by_k)$, i.e., for any permutation $\sigma$, 
\begin{align} \label{eq:equi-inv property}
  Q^\star(\sigma(s_k)) = Q^{\star}(\sigma_{k}(\bx), \sigma_{N-k}(\by)) = \sigma_{N-k} (Q^{\star}(s_{k})). \end{align}
\end{prop}
The EI property of our IS-MDP plays a critical role in reducing the state space for IS-MDP, i.e., ignore the redundant states through permutations.
\end{comment}


%\note{interpretation as a symmetry. }

\begin{comment}
In this subsection, we induce a symmetry called EI property in the optimal action-value function  $\tQ^{\star}(\ts, \ta)$.
We found permutation invariant property of the transitions in IS-MDP \eqref{eq:tranGREEDYSEL}. 
Recall that state $\ts_{k}:=(\tbx, \tby)$ can be represented as a tuple of sets where $\tbx:=\{x_{1}, \cdots, x_{k}\}$ and $\tby:=\{y_{1}, \cdots, y_{N-k}\}$ for $k=0, \cdots, K-1$.
The order of the items in $\tbx$ or  in $\tby$ does not affect to the state $\ts_{k} = (\tbx, \tby)$, i.e.,
for any permutations of $k$ and $N-k$, $\sigma_{k}\in \bS_{k}$ and $\sigma_{N-k } \in \bS_{N-k}$ respectively, we define $$\sigma_{k}(\bx):=\{x_{\sigma_{k}(1)}, \cdots, x_{\sigma_{k}(k)}\}, \qquad \sigma_{N-k}(\by):=\{y_{\sigma_{N-k}(1)}, \cdots, y_{\sigma_{N-k}(N-k)}\}. $$ 
Furthemore, we set 
$\sigma(\ts_{k})$ as 
\begin{gather} \label{eq:sigma_s}
   \sigma(\ts_{k}) := ( \sigma_{k}(\tbx), \sigma_{N-k}(\tby)). 
\end{gather}
% \begin{align} \label{eq:sigma_s}

% \end{align}
The following state-action pairs $(s_{k}, a_{k})$ and $(\sigma_{s_{k}}(s_{k}), \sigma_{N-k}(\tby))$ shares the same reward and transition probability function, i.e.,
\begin{align} \label{eq:tranGREEDYSEL}
 & \cR(s_{k}, a_{k}) = \cR(\sigma(s_{k}),  \sigma_{N-k}(a_{k})), \quad
\cP(s_{k} ', \tr \mid s_{k}, a_{k})) = \cP(s_{k} ', \tr \mid \sigma(s_{k}),  \sigma_{N-k}(a_{k}))). 
\end{align}

Now, we can derive the EI property of the optimal action value function $Q^{\star}(s_{k})$ from the symmetry in \eqref{eq:tranGREEDYSEL}. For convenient connected to our DQN design in Section \ref{sec:greedy-select-dqn}, we define the optimal action value functions as \begin{align} \label{eq:Qvalueopt}
[\tQ^{\star}_{k}(\ts_{k})]_{i\in \by, c \in \cC}:= \tQ^{\star}_{k}(\ts_{k}, (i, c) ).  
\end{align}
\begin{prop} [Equi-Invariant Property]
  \label{prop:ei_optimal}
If we follow the above definition of $Q^{\star}_{k}(\ts_{k})$, 
for all $\sigma_{k}$ and $\sigma_{N-k }$, 
\begin{equation} \label{eq:equi-inv property}
  \tQ_{k}^{\star}(\sigma_{k}(\tbx),  \sigma_{N-k}(\tby)) =  \sigma_{N-k } (\tQ_{k}^{\star}(\ts_{k})).  
\end{equation}
We will say that  function $F$ has  \textit{permutation Equi-Invariant property} to the $\tby$ and $\tbx$ (EI property) if $F$ satisfies \eqref{eq:equi-inv property}. 
\end{prop}
EI property is very powerful property in reducing number of state-action pairs by ignoring the permutations of the orders of the items. 
In the next section, we will present our DQN algorithm and our neural network architecture with the EI property to exploit this property.
The general relationship of symmetries between the transition functions and the optimal value functions were studied by 
\citet{zinkevich2001symmetry}.
Our proposition with EI property in the optimal q-functions can be regarded as a special case of their works.
\end{comment}


\subsection{IS-DQN}
\label{sec:greedy-select-dqn}
\subsubsection{Cascaded Q-networks}
Recall Section \ref{sec:greedy-select-dqn} that the optimal Q-functions $Q^{\star}(s_{k})$ have different input state dimensions and  output action-value dimensions since the dimensions of p-state $s_k = (\bx_{k}, \by_{k})$ and coupled action sets  $\set{A}_k(s_{k}) = \{ (i,c) \mid i \in \by_{k}, c \in \cC \} $ vary as $k$ changes.
Introducing IS-MDP to our problem makes the Q-function at phase $k$ endowed with different dimensions of input and output vectors for each phase $k,$ i.e., the phase-$k$ Q-function $Q_k: \set{S_k} \mapsto \real^{N-k} \otimes \real^{\vert \cC \vert}.$ 

This motivates us to build $K$ cascaded Q-networks $[\tQ(\ts_{k};\omega_k)]_{k=0}^{K-1}$, as illustrated in Figure~\ref{fig:Perphase_networks}.
With these cascaded Q-networks, there are $k$-phase loss functions $l_{k}(\omega_{k})$ for each phase $k$ for transition $(s_{k}, a_{k}, r_{k}, s_{k+1})$ are also defined:
% One difficulty to design a single network $\tQ(\ts;\omega)$ for IS-MDP is that both input and output dimensions of $\tQ(\ts_{k};\omega)$ are different for various values of $k$.
% Therefore, we propose to use $K$ separate neural networks $\tQ_{k}(\ts_{k} ; \omega_{k}), 0 \leq k < K$ for $K$ different dimensions of state $s_{k}$. 
% Figure~\ref{fig:Perphase_networks} illustrates how these $K$ networks work.
% During selecting a $K$ combinated action $a=\{(n_{1},c_{1}), \cdots, (n_{K}, c_{K}) \}$, 
% for each phase $k$, each $Q_{k}$ selects the $k^{th}$ pair of $\{$item, command$\}$ only and transfers the next intermediate state $s_{k+1}$ to the next Q-network $Q_{k+1}$.
% This process goes until the last $Q_{K-1}$ selects its $(K-1)^{th}$ pair.
% The divided $K$ phase are saved in the replay buffers. 
% The loss function $L_{k}(\omega_{k})$ is also  defined with the consideration of the fact as follows:

%% previous equation 12/31
% \begin{compactenum}[(i)]
% \item for $0 \leq k \leq K-1,$
% \begin{multline} \label{eq:loss_k}
% l_{k}(\ts_{k}, \ta_{k}, 0, \ts_{k+1}  ; \omega_{k}):= \cr 
% \left (\tQ_{k}(\ts_{k},\ta_{k};\omega_{k}) - (0 + 1 \cdot \max_{\ta_{k+1} \in \tcA_{k+1}(\ts_{k+1})} 
%     \tQ_{k+1}(\ts_{k+1},\ta_{k+1};\omega_{k+1} ')) \right)^{2},
% \end{multline}
% \item for $k=K-1,$
% \begin{multline} \label{eq:loss_K-1}
% l_{K-1}(\ts_{K-1}, \ta_{K-1}, r, s'  ; \omega_{K-1}):= \cr 
% \left (\tQ_{K-1}(\ts_{K-1},\ta_{K-1};\omega_{K-1}) - (\tr  + \gamma \max_{\ta ' \in \tcA_{0}(\ts')} 
%     \tQ_{0}(\ts ',\ta ';\omega_{0} ')) \right)^{2}.
% \end{multline}
% \end{compactenum}
  \begin{compactenum}[(i)] 
    \item for $0 \leq k < K-1,$
    \begin{multline} \label{eq:loss_k}
    l_{k}(s_{k}, a_{k}, r_{k}, s_{k+1}):= \cr 
    \left (\tQ_{k}(\ts_{k},\ta_{k}) - \max_{\ta_{k+1} \in \tcA_{k+1}} 
        \tQ_{k+1}(\ts_{k+1},\ta_{k+1}) \right)^{2},
    \end{multline}
    \item for $k=K-1,$
    \begin{multline} \label{eq:loss_K-1}
    l_{k}(s_{k}, a_{k}, r_{k}, s_{k+1}):= \cr 
    \left (\tQ_{k}(\ts_{k},\ta_{k}) - (\tr  + \gamma \max_{\ta ' \in \tcA_{0}}
        \tQ_{0}(\ts ',\ta ')) \right)^{2}.
    \end{multline}
    \end{compactenum}

% \begin{align*} 
%    k <K-1: \quad & L_{k}(\ts_{k}, \ta_{k}, 0, \ts_{k+1}  ; \omega_{k}):= (\tQ_{k}(\ts_{k},\ta_{k};\omega_{k}) - (0 +  \max_{\ta_{k+1} \in \tcA(\ts)} 
%     \tQ_{k+1}(\ts_{k+1},\ta_{k+1};\omega_{k+1} ')))^{2},\\ 
%     k = K-1: \quad & L_{K-1}(\ts_{K-1}, \ta_{K-1}, r, s'  ; \omega_{K-1}):= (\tQ_{K-1}(\ts,\ta;\omega) - (\tr  + \gamma \max_{\ta ' \in \tcA(\ts)} 
%     \tQ_{0}(\ts ',\ta ';\omega_{0} ')))^{2}. 
% \end{align*}
The above definition is a conversion of the loss function $L_{\omega}$ in \eqref{eq:loss_general} for general DQN. 
We differentiate the main Q-network $Q_{k}$ for current p-state $s_{k}$ from the target Q-network $Q_{k+1}$ for the next p-state $s_{k+1}$. 
% The phase $k=K-1$ also can be handled  similarly.
We set the discount factor equals to $\gamma$ only at final phase $K-1$ and set $1$ in the remaining cases for $k<K-1$. 
This is not strictly necessary, but we guess this method would help the inter-sharing among the cascaded Q-networks   described in Section \ref{sec:Intersharing}.
% is updated using the transition experience $(\ts_{k}, \ta_{k}, \tr, \ts_{k+1})$ sampled from the $k^{th}$ replay buffer.

\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.9\linewidth]{figure/Perphase_networks}
  \caption{Simple example of per-phase Q-networks $Q_{k}$s and the loss function $l_{k}$s when $K=3, N=4$.  
% There are $K$ different simplified per-phase Q-networks. 
 The loss function $l_{k}$ is defined between p-state $s_{k}$ and $s_{k+1}$ since every transition from $\cS_{k} \rightarrow \cS_{k+1}$. 
 In I-sharing in Section~\ref{sec:EINET}, the weights with the same color per each Q-network $Q_{k}$ have the same values. If U-sharing in Section~\ref{sec:Intersharing}, all the same colored weights even in different Q-networks also share the weight value with some normalizings.}
  \label{fig:Perphase_networks}
\end{figure*}
 
It is true that IS-DQN requires $K$ distinct Q-networks and the size of each Q-network grows as the number of the item $N$ increases.
This fact can be problematic in scalability when $N$ or $K$ is large.
In the following sections, we propose a novel two-levels of parameter sharing, which overcomes such weakness, which is one of our key contributions of this paper.
In Section \ref{sec:EINET}, we suggest a first level of parameter sharing for each $Q_{k}$ which called intra-sharing. 
In Section \ref{sec:Intersharing},  we suggest an second level of parameter-sharing between the distinct $Q_{k}$s for all $k = 0,1, \cdots, K-1$. 

% as $K$ grows and requires large number of parameters when $N$ is large,
% which induces large computation cost, overfitting, and slow convergence.
% To handle both large $N$ and $K$, we present two parameter sharing methods:
% intra-parameter sharing (Section~\ref{sec:EINET}) and
% inter-parameter sharing (Section~\ref{sec:Intersharing}).

% \vspace{-0.2cm}
\subsubsection{Intra-Parameter Sharing}
\label{sec:EINET}
%% previous figure
% \begin{wrapfigure}[11]{R}{.55\textwidth}
%   \vspace{-12pt}
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \begin{minipage}{.8\textwidth}
%         \includegraphics[width=\linewidth]{figure/layer-a}
%       \end{minipage}
%       \caption{Layer $\phi_A$}
%       \label{fig:layer-a}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \begin{minipage}{.8\textwidth}
%         \includegraphics[width=\linewidth]{figure/layer-b}
%       \end{minipage}
%       \caption{Layer $\phi_B$}
%       \label{fig:layer-b}
%     \end{subfigure}
%     \caption{Two layers for intra-parameter sharing. The parameters with the same color share the same value.} \vspace{-0.2cm}
%     \label{fig:eilayers}
%   \end{wrapfigure}

  \begin{figure}
    \includegraphics[width=\linewidth]{figure/EINET}
        % \end{minipage}
      \caption{Simlple Intra-Sharing Q-network $Q_{k}$ with two layers. The same colored edges in the same layer are tied together.}
      \label{fig:eilayers}
    \end{figure}


We first present \textit{intra-parameter sharing} (I-sharing)  that is used for each cascaded Q-network $Q_k$ at phase $k$ which always satisfies EI so the network can exploit EI in \eqref{eq:equi-inv property} or $Q_{k}(\sigma(s_{k}))=\sigma_{y}(Q_{k}(s_{k}))$.
In other words, $Q_k$ with I-sharing correctly estimates the action values which are not depended by the orders of the items in $\bx_{k}$ or $\by_{k}$.
From now on, we will denote the $Q_{k}$ as the cascaded Q-network with I-sharing. 
% The key feature in this parameter sharing is about proposing a new neural network architecture 
% that exploits a mixture of invariance and equivariance, formalized in Proposition~\ref{prop:ei_optimal} or \eqref{eq:equi-inv property}.
% \note{HS: recall that the output $Q_k$ }
The I-shared Q-network $Q_{k}$
 is composed  of two parameter-shared layers $\phi_{k}^{A}$ and  $\phi_{k}^{B}$ which $\phi_{k}^{A}$ and  $\phi_{k}^{B}$ satisfies special permutational properties so $Q_{k}$ also satisfies EI.  
The layers $\phi_{k}^{A}$ are stacking up multiple times and the layer $\phi_{k}^{B}$ is only used as the last output layer in $Q_{k}$. 
The simple form of $Q_{k}$ is described in Figure \ref{fig:eilayers}.
Under the fact that the same colored weights in the same layer are tied together, the layer $\phi_{k}^{A}$ preserves the orders of both the selected items $\bx$ and  unselected items $\by$ while the layer $\phi_{k}^{B}$ preserves the order of the only selected items in $\by$. Therefore, $Q_{k}$ preserves the order of the items in $\by$ (permutation equivariant) and equally treats the selected items in $\bx$ (permutation invariant).

To explain more specifically why $Q_{k}$ satisfies EI, firstly consider the relationship between the input nodes and output nodes in  $\phi_{k}^{A}$. For example, suppose that the order of the nodes $x_{1}, x_{2}$ is changed, the order of the output nodes $h_{1}^{x}, h_{2}^{x}$ would also be changed while other nodes maintain their values. 
However, even though $h_{1}^{x}, h_{2}^{x}$ are changed, the output q-values of layer $\phi_{k}^{B}$ does not depend from the change or implies that $Q_{k}$ is  permutation invariant to $\bx$ with the permutation $\sigma_{x}$. 
On the other hand, if the orders of $y_{1}, y_{2}$ change, both $h_{1}^{y}, h_{2}^{y}$ and $q_{1}, q_{2}$ follow this change which implies that $Q_{k}$ is permutation equivariant to $\by$ with the permutation $\sigma_{y}$, i.e., $\forall \sigma = (\sigma_{x}, \sigma_{y}) \in \bS_{k} \otimes \bS_{N-k}, $
\begin{align} \label{eq:layersymmetry}
  \begin{split}
   \phi_{k}^{A}(\sigma(\ts_{k}))= \sigma(\phi_{k}^{A}(\ts_{k})), \quad
    \phi_{k}^{B}(\sigma(\ts_{k})) = \sigma_{y}(\phi_{k}^{B}(\ts_{k})) 
    \\
     Q_{k}(\sigma(\ts_{k})) = \sigma_{y}(Q_{k}(\ts_{k})).
  \end{split}
  \end{align}
The layer $\phi_{k}^{A}$ can be regarded as  equivariant both $\bx, \by$ while $\phi_{k}^{B}$ is only equivariant to $\by$.
In $Q_{k}$, all the layers except the output layer has structure of $\phi_{k}^{A}$ and the final output layer has structure of $\phi_{k}^{B}$ or  $Q_{k}:=\phi_{k}^{B} \circ \phi_{k}^{A} \circ \cdots \circ \phi_{k}^{A}.$ 
It is easily induced from \eqref{eq:layersymmetry} that $Q_{k}$ satisfies EI. 
For presentational simplicity, in Figure \ref{fig:eilayers}, we simlify the case when $\bx_{k} \in \Real^{k}$, $\by_{k} \in \Real^{N-k}$ and $\vert \cC \vert =1$. The complete description of our intra-sharing will be given in Appendix \ref{sec:IntraSharing}.

The intra-sharing is very efficient to handle when the number of item $N$ is large. 
% It reduces a lot of weight parameter with the from th 
It only has the number of weights $O(K)$ compared to the same architecture neural network without sharing requires $O(N^{2}K)$ number of parameters. 
However, it still have some problems when $K$ grows, since there would be $K$ cascaded Q-networks $Q_{k}(s_{k})$ exists. 
In the following section, we shares additional parameters among $K$ cascaded Q-networks by inter-sharing method.

% Therefore, the $Q_{k}(\bx_{k}, \by_{k}): \Real^{k} \otimes \Real^{N-k} \rightarrow \Real^{N-k}$ where the $j$th element in the output vector implies the action values for $y_{j}$.


% \begin{align} \label{eq:layersymmetry}
%   \phi_{k}^{A}(\sigma(\ts_{k}))= \sigma(\phi_{k}^{A}(\ts_{k})), \quad
%     \phi_{k}^{B}(\sigma(\ts_{k})) = \sigma_{N-k}(\phi_{k}^{B}(\ts_{k})).
%    \end{align}

% As a result, $Q_{k}$ also always satisfies EI to $(\bx, \by)$ if we set $Q_{k}:=\phi_{k}^{B} \circ \phi_{k}^{A} \circ \cdots \circ \phi_{k}^{A}$.



% In this subsection, we explain the intra-parameter shared neural network architectures to approximate the optimal Q-functions $\tQ^{\star}_{k}(\ts_{k})$ with EI property in \ref{eq:equi-inv property}. 
% The intra-parameter sharing makes to have the EI property to the networks.
% We first define two types of fully connected layers $\phi^{A}, \phi^{B}$ with the idea of {\em parameter sharing} and then combine multiple layers to make a deep neural network.  

% and prove the local minimal parameter in the EINET is also the local minimal parameter in a same-architectured deep neural network without any parameter sharing. 

%\smallskip \noindent {\bf Intra-Parameter Shared Layers.} 
%\myparagraph{Intra-Parameter Shared Layers} 


% We first present the simplest version of intra-parameter sharing method with single layers.
% We will present detailed explanation of intra-parameter sharing such as with multiple channels in the Appendix \ref{sec:multiplechannels}.


% \note{The following should be explained. Why we need two types of layers. What's the role of each layer? How are you connect them to make the final deep network? How many parameter reduction occurs?

% Reviewer's mind: They want to understand how well equivariance and invariance are realized in a mixed manner. They are ready to be surprised by our smartness, but we failed to surprise them.}



% We define two types of fully connected layers $\phi_{k}^{A}, \phi_{k}^{B}$ called intra-parameter shared layers.
% The basic architectures are elaborated in Figure~\ref{fig:eilayers}. The same colored weight parameters are tied together. 
% The key intuition of intra-parameter sharing method is that shared the parameters so the layers have the EI property or do not be affected by the orders of the items such as $x_{j} \in \bx$ or $y_{j} \in \by$.
% There are two types of layer 
% $\phi_{k}^{A}: \Real^{k} \otimes \Real^{N-k}  \mapsto \Real^{k} \otimes \Real^{N-k} $ and
% $\phi_{k}^{B}: \Real^{k} \otimes \Real^{N-k}  \mapsto \Real^{N-k} $ with the following property for any $\sigma_{k}(\bx)$,  $\sigma_{N-k}(\by)$, and $\sigma(s_{k})$ defined in \eqref{eq:sigma_s},
% %  \begin{align} \label{eq:layersymmetry}
% % \phi_{k}^{A}(\sigma(\ts_{k}))= \sigma(\phi_{k}^{A}(\ts_{k})), \hspace{0.15cm}
% %   \phi_{k}^{B}(\sigma(\ts_{k})) = \sigma_{N-k}(\phi_{k}^{B}(\ts_{k})), \hspace{0.15cm}  G(\ts_{k})= \phi_{k}^{B} \circ \phi_{k}^{A} \circ \cdots \circ \phi_{k}^{A}(\ts_{k}).
% %  \end{align}
%  The deep neural network $G(\ts_{k})$ is made up of composition of layers always satisfies EI property in \eqref{eq:equi-inv property}.
%  The detailed explanation of the layers are described in the appendix \ref{sec:IntraSharing}. 
%  This intra-parameter sharing is very efficient to handle when $N$ is large since the parameter sharing ignores the orders of the items in $\bx$ or $\by$. However, it still have some problem when $K$ grows, since there would be large number of $Q_{k}(s_{k})$ exists. 
%  In the following section, we shares additional parameters among $K$ cascaded Q-networks.


\subsubsection{Inter-Parameter Sharing}
\label{sec:Intersharing}
% \note{What Reviewers want to know: (i) what is inter-parameter sharing? (ii) Why does it make sense? What intuition is working here? (iii) What's the expected weakness of this mehtod, and why is it expected to be insignificant? (iv) How many parameter reduction occurs? Thus, the total reduction from that without parameter sharing to that with intra- and inter-parameter sharing?}
In this subsection, we propose second-level parameter sharing methods among cascaded Q-networks after I-sharing called \textit{unified-parameter sharing} (U-sharing) and \textit{progressive-parameter sharing} (P-sharing). 
In I-sharing, the cascaded Q-Networks share similar network architectures with the same number of weight parameters regardless of phase $k$.
As an example in Figure 2, the whole  cascaded Q-networks for any phase consist of two weight parameters marked in orange and green.
In I-sharing, each cascaded Q-networks do not share its own weight parameters with others. 
However, we conjecture that there are  some similarities among weight parameters of the cascaded Q-networks. 
The intuition arises from that 
selecting the same item at a certain phase does not effect to expected reward of IS-MDP. 
Therefore, the criteria for item evaluation would be similar at any phase.

% However, in intra-sharing, the parameters in different Q-networks $Q_{k}$ and $ Q_{k'}$ are not tied together so the total number of the parameters $O(K)$. 
% For example, There are 3 cascaded Q-network $Q_{0}, Q_{1}, Q_{2}$ in Figure~{\ref{fig:Perphase_networks}}.
% In inter-sharing, the whole green edges in $Q_{0}, Q_{1}, Q_{2}$ share the one fixed value while there are 3 different values for green edges for each network in intra-sharing.

% In Q-network, the weight parameters decide how to intepret the information of input nodes.
% For example, the orange lines decides the role of the already selected items $x$'s information to estimate q-values.
% The inter-sharing is based on conjecture that these interpretation roles does not change much as the number of already selected items $k$ varies.
% Although this conjecture would not be always true, but it is natural in many IS-MDP models even when the agent should consider the complex combinatorial selection effects.

In U-sharing, we use this similarity at an extreme level by making whole cascaded Q-networks share a single parameter set with properly scaled weight parameters depending phase $k$.
The detailed scaling method is explained in appendix \ref{sec:IntraSharing_math_single_channel}.
Therefore, the number of the weight parameters are reduced from $O(K)$ in I-sharing to $O(1)$ in U-sharing.
The benefit of U-sharing is that a given experience at a specific phase $k$ can be used to update not only the corresponding cascaded Q-network $Q_{k}$ but also the other cascaded Q-networks for different phases simultaneously.
This enables sample-efficient updates of the overall cascaded Q-networks.
There is an expected weakness of U-sharing: decrease in expressive power of the cascaded Q-networks from the restriction of weight parameters.


To combine both advantages of I-sharing and U-sharing, we propose P-sharing.
While training with P-sharing, we start with a single parameter set and then progressively increase the number of the weight parameter sets doubly until it reaches $K$.
The Q-networks with nearby phases tends to share the same parameter set longer until the number of the parameter set increases enough.
The Q-Networks with nearby phases tends to share the same parameter set longer until the number of the parameter set increases enough.
The detail is visualized in Figure 3.
In the early stage of the learning where the networks are not stable, the Q-networks are trained sample-efficiently as they exploit the advantages of U-sharing.
On the other hand, as the training progresses gradually, the Q-networks are able to be trained more elaborately by increasing the number of the weight parameter sets.
In P-sharing, the number of the total weight parameters increases from $O(1)$ to $O(K)$ during training.

\begin{figure}[ht]
  \centering
  \includegraphics[width=.99\linewidth]{figure/Progressive_learning.pdf}
  \caption{Simple scenario for progressive-sharing when $K=4$. At the initial training, whole intra-shared Q-networks are generated from a single parameter set $Par_{0}$ which is the same way as U-sharing. After a certain training step, the parameter set is divided into two paraemeter set $Par_{0}$ and $Par_{2}$ which are used to construct Q-network $Q_{0}, Q_{1}$ and $Q_{2}, Q_{3}$  respectively.  Finally, each Q-networks $Q_{k}$ has its own weight parmaeter set $Par_{k}$ respectively for all $k \in \{0,\cdots,3 \}$.}
  \label{fig:Progressive_learning}
\end{figure}

%% Previous writing before 12/25
% There are two advantages of inter-sharing when $K$ grows.
% Firstly and most importantly, inter-sharing helps the cascaded Q-networks updates their q-values much more efficiently by sharing the parameters.
% Suppose that we use only intra-sharing method.
% When we update the cascaded Q-networks, only $Q_{K-1}$ updates its network with non-zero reward in the loss $l_{K-1}$ in \eqref{eq:loss_K-1}.
% Which means the other networks $Q_{0} \sim Q_{K-2}$ should wait until $Q_{K-1}$ learns some meaningful q-values. 
% This updates cascades from $Q_{K-2}, \cdots, Q_{0}$ one by one.
% Therefore, it will takes some time until that these updates cascades to the last network $Q_{0}$.
% However, when we use inter-sharing, the other networks $Q_{k}$ for $0\leq k \leq K-2$ can be simultaneously updated when the agent just reduces the loss in $l_{K-1}$. 
% The faster update of $Q_{0}$ would help  to update $Q_{K-1}$ again since $Q_{0}$ generates the target values in $l_{K-1}$ for given experience.
% Secondly, a small number of the parameters reduces the memory and computation cost during the gradient descent of the networks. 
% For example, the numbers of parameters for IS-MDP(K,N) are $O(N^{2}K), O(K)$, $O(1)$ as we do not use any parameter sharing, using intra-sharing only, and inter-sharing method respectively.
% Furthermore, thanks to algorithms in tensorflow that increase the computation speed a lot when we use inter-sharing.
% The simulation results in Section \ref{sec:eval} strongly show both advantages of our inter-sharing method.

% In Figure~{\ref{fig:Perphase_networks}}, each $Q_{k}$ has some similar shapes and fixed number of parameters. For example, the yellow dot lines in $Q_{1}(s_{1})$ and $Q_{2}(s_{2})$ may have similar role to transfer the information (item, command) of the selected elements $x_{1}, x_{2}$. 


% In inter-parameter sharing, the whole $Q_{k}$ shares the same weight value  with some normalization rule by specific $N,k$.
% By making this way, the number of the weight parameters in inter-parameter sharing methods  do not be affected by varying $K$.
% Furthermore, this inter-parameter sharing method facilitates  fast convergence of the training since each $Q_{k}$ shares their knowledge directly each others.

% In normal DQN case, the trained network would be useless when the size of $N$ differs. 
% In our DQN algorithm with the similar manner to the intuition for inter-parameter sharing, the trained parameter of this network may be reused in another environment with different input dimension, such as $N=200$.




% In the previous EI-NN, $\ovt(x,y): R^{1} \rightarrow R^{1}$ are assigned between the $x_{i}$ and $h_{j}^{1,y}$. 

% from $H_{\ovt} : R^{N+M} \rightarrow R^{M}$ to   $H_{\ovt} : R^{NK_{I}+MK_{E}} \rightarrow R^{M\times K_{O}} $ where $K_{I},K_{E}$, and $K_{O}$ is the number of the dimension for each elements $x$, $y$, and 


% which handles the case when the input elements $x$ or $y$ have multiple features as well as the output of the policy $\pi$ 
% %  All nodes in the neural network can be regarded as $k$ dimensional vector rather than a simple $1$-dimensional value where $k$ is an arbitrary positive integer.  
% The first layer $ \phi^{1}:R^{N+M} \rightarrow R^{N+M} $ of neural network $G_{g(\ovt)}$ can be extended to  $ \phi^{1}:R^{(N+M)\times K_{0}} \rightarrow R^{(N+M)\times K_{1}} $ where $K_{0},K_{1}$ is the number of the 
% The shared weight parameters in $G_{g(\overline{\omega})}$ are also converted from $1$-dimensional value to proper dimensional matrix.
% %  such as $w_{x,y} ^{1,g}$ 
% For example, suppose that the invariant input elements $\bx_{i}$ has $k_{x}$ dimensional vector and the hidden node $\bh_{j}^{1,y}$ has $h_{y}$ dimensional vector. 
% In this case, we can extend the $1$-dimensional weight parameter $w_{x,y} ^{1,g}$ to $h_{y} \times k_{x}$-dimensional matrix weight parameters $\bw_{x,y}^{1,g}$.   
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> figure/evaluation.tex <==
\section{Experimental Setup} \label{sec:eval}

%\noindent {\bf Tasks} 

% need to explain two tasks as a sequential combinatorial selection problem.
%
% We compare the performance of ISQ in aformentioned tasks with a rule-based heuristic and variants of DQN \note{refs}. 
%
%\note{need to explain the idea of baseline algorithms for comparison: a rule-based heuristic and RL algorithms, with references: key difference of those baseline algorithms compared to ours.}. 

% hyperparameters: type of optimizer, learning rate, batch size, target network update frequency, and replay buffer size. 


\subsection{Environments} 
To evaluate ISQ, we consider two different tasks: Circle Selection (CS) which is a synthetic
environment we made for a demonstrative purpose, and Selective Predator and Prey
(PP) which is a modified version of Predator and Prey  in \cite{stone2000multiagent} for multi-agent
reinforcement learning problem.

\smallskip\noindent{\bf Circle Selection (CS)} \label{sec:exp-CS} 
In this task, there are randomly moving $N+U$ circles on a two-dimensional Euclidean plane, where the radius of each circle increases randomly with a constant ratio. We consider that only $N$ circles are selectable, while the other $U$ circles are unselectable. At every time, the agent observes a position of each circle's center and its radius as a state $s$, and should select $K$ circles among $N$ selectable ones and move each selected circle a fixed distance in one of the five commands for directions: {\em up, down, left, right} and {\em stay} - as an action. 
After the action, the agent receives reward r which is a summation of values for each selected circle which is moved by the command. 
The value is given as a negative value of the circle’s area or zero if the circle overlaps to some of the $U$ unselectable circles (\ref{fig:negative}) or some of the other $K-1$ selected circles (\ref{fig:zero}), respectively, while it is given as a positive reward otherwise (\ref{fig:positive}).
The agent should avoid the overlapping by carefully choosing the commands of the selected circles. 
Some examples scenarios are described in Figure~\ref{fig:circles}.
% \note{example of the three different rewards, in case of one circle selection.} 
After that, all selected $K$ circles and any unselectable circle overlapping to them are replaced with new circles, which are initialized at random locations with small initial radius. 
% Q: when the episode terminates?



\smallskip\noindent {\bf Selective Predator-Prey (PP)} 
In this task, multiple predators should capture randomly moving preys. 
The agent observes the positions of the whole predators and whole preys in a 2-dimensional grid world. 
The  agent selects $K$ predators (which are items in SELECT-MDP) and allocates one of the 5 commands to each predator: \textit{`stay', `up', `right', `left', `down'}.   
The only selected predators can move and capture the preys. 
The reward of the action is the number of preys which are caught by the selected predators. 
Prey is caught if and only if two or more selected predators catch the prey at the same time. 


\begin{figure}
  \centering 
  \subfloat[$r<0$]{\label{fig:negative}\includegraphics[width=0.32\linewidth]{figure/circle_negative}}
  \subfloat[$r=0$]{\label{fig:zero}\includegraphics[width=0.32\linewidth]{figure/circle_zero}}
  \subfloat[$r>0$]{\label{fig:positive}\includegraphics[width=0.32\linewidth]{figure/circle_positive}}
  \caption{Example scenarios of Circle Selection (CS) task with $N=3$, $U=1$, $K=2$ from the common state.
  Circles with an orange line or green dashes are selectable or unselectable, respectively.
  The shaded circles are the selected circles and the arrow represents the commands. 
 (a) Both selected circles overlap to the unselectable circles.
 The negative value of the summation of the area of each selected circle becomes the reward.
  (b)
  Both selected circles do not overlap to the unselectable circle from the commands, but they still overlap each other. The reward $r$ becomes zero. 
  (c) Both selected circle do not overlap to any other selected circles or unselectable circle. So the reward is positive.  
  }  
  \label{fig:circles}
\end{figure}


\subsection{Tested algorithms and Hyperparameters}
\smallskip\noindent {\bf Tested algorithms} 
As described in Section~\ref{sec:greedy-select-dqn}, we compare three versions of ISQ with intra-sharing only (ISQ-I), unified-sharing (ISQ-U), progressive-sharing (ISQ-P). 
As baselines, we compare with a vanilla DQN \cite{mnih2015human} and a sorting DQN, which reduces a state space by sorting the order of items based on a pre-defined rule before applying a vanilla DQN.
We develop a myopic DQN which is similar to ISQ and maximizes the reward in the next step.   
This myopic DQN represents many other RL or combinatorial MAB algorithms in combinatorial selection algorithms which do not consider future state after the combinatorial action \cite{qin2014contextual,wen2015efficient,chen2018contextual,li2016contextual,kool2018attention,dai2017learning}.  
We also modify two value-based MARL algorithms for fully cooperative tasks: Independent DQN (IDQN) \cite{tampuu2017multiagent} and Random-Select DQN (RSQ) \cite{usunier2016episodic}.
In IDQN, each item observes the whole state and has its q-function where the action space equals to $\cC$. 
The agent selects top $K$ items with the highest q-values. 
The only selected items' q-functions can be updated with the shared reward.
RSQ is almost the same to ISQ except the agent selects  a item uniform randomly and evaluates a small number of the action-values for commands for the selected item.
It is known that RSQ can achieve the opitmal policy for general fully cooperative MARL or SELECT-MDP with $N=K$ \cite{usunier2016episodic}. 

% In particular, it chooses $K$ largest non-overlapped selectable circles at every time, maximizing the {\em instant} reward at the next state.
\smallskip\noindent {\bf Setup} 
We train models in tasks mentioned above and evaluate them by averaging rewards without any exploration during $20$ independent episodes.  
The shaded area in each plot indicates  95$\%$ confidence intervals on $4$ trials with different seeds. 
We use the same hyperparameters for all tasks except for the numbers of total training steps. 
We use a replay buffer whose size is $50,000$, a learning rate with $0.001$,  minibatch whose size with $32$, Adam optimizer \cite{kingma2014adam}, a discount factor with $0.99$, the target network update frequency with $1000$, $\epsilon$-greedy exploration with $0.1$ lower bound, $3$-hidden layers whose numbers of nodes are $4$ times higher than the number of input nodes. 
The detailed codes and settings are uploaded at github \note{github link}.  
\section{Results}
\begin{figure*}[ht] 
  \centering
  \subfloat[$N=5$]{\includegraphics[width=0.33\textwidth]{figure/circle_K-1_conf-graph_ne-5}}
  \subfloat[$N=20$]{\includegraphics[width=0.33\textwidth]{figure/circle_K-1_conf-graph_ne-20}}
  \subfloat[$N=50$]{\includegraphics[width=0.33\textwidth]{figure/circle_K-1_conf-graph_ne-50}}
  \caption{Learning curves for Circle Selection when $K=1$ and $\vert \cC \vert = 1$. Each episode consists of 2500 steps. 
  % When $N$ is small, all the baseline DQNs perform similar. 
  % However, as $N$ grows,   
  % the performance of vanilla DQN fails to learn a meaningful policy. Sorting DQN learns a policy which is better than the random policy but the gap between I-sharing DQN grows as $N$ grows. 
  \note{better to use the same y-range in all three subfloats} } 
  \label{fig:learning-circle-1}
\end{figure*} 
\subsection{Single Item Selection ($K=1$)}
We first check the power of intra-parameter sharing (I-sharing) when the number of items $N$ grows. 
We perform experiment in simple CS tasks with a single unselectable circle, i.e., $K = 1, |\mathcal{C}| = 1$ and $U = 1$. 
Under this tasks, we compare ISQ to the baseline RL algorithms without intra-parameter sharing as well as a sorting DQN which is same as the vanilla DQN, but the state is sorted based on a pre-defined rule, so the agent does not need to explore the $N!$ equivalent states. 
We sort the circles in radial order which seems essential features in CS.

% \smallskip\noindent{\bf Impact of intra-parameter sharing} 
\subsubsection{Impact of intra-parameter sharing} 
% To solely demonstrate the impact of I-sharing, we compare with a vanilla DQN (\note{ref}) and a sorting DQN, which reduces a state space by sorting the information of items based on a pre-defined rule before applying a vanilla DQN. 
Fig.~\ref{fig:learning-circle-1} illustrates the learning curves of these schemes over $175 \cdot 10^{4}$ training steps for $N = 5, 20$, and $50$. 
The whole baselines without any consideration of the symmetry in SELECT-MDP fail to learn good policies especially when $N=50$ (Vanilla DQN, MQ, RSQ). 
We omit IDQN since IDQN is the same as vanilla DQN when $K=1$. 
This fact strongly suggests that the state space becomes too large to be explored as $N$ grows. 
Compared to the vanilla DQN, the sorting DQN learns some meaningful policies under large $N$ by reducing the state space. 
However, even though both sorting DQN and ISQ equally exploit the symmetry, ISQ still performs similarly when $N$ is small and outperforms when $N$ is large.
It supports our analytical findings in Theorem~\ref{thm:local optimal} and Theorem~\ref{thm:universal} in that the idea of intra-sharing does not degrade any representation power although it reduces the number of the weight parameters from $O(N^{2})$ to $O(1)$. 
Furthermore, we guess that too many weight parameters generate the inefficiency of the training Q-networks which is the reason that ISQ outperforms sorting DQN as $N$ grows.


% As a result, to maximize the long-term reward, one should (i) select
% non-overlapping circles among $N$ circles, (ii) make the selected
% circles move in proper directions to avoid overlapping, and (iii)
% wait some circles to grow. 

\begin{figure*}[ht]
  \centering
  \subfloat[$N=50,K=6$]{\label{fig:k6n50}\includegraphics[width=0.33\textwidth]{figure/circle_K-6_conf-graph_ne-50.pdf}}
  \subfloat[$N=200,K=6$]{\label{fig:k6n200}\includegraphics[width=0.33\textwidth]{figure/circle_K-6_conf-graph_ne-200.pdf}}
  \subfloat[Distribution for Radius of selected circles ]{\label{fig:HeurvsPsharing}\includegraphics[width=0.33\textwidth]{figure/radius_selected}}
  \caption{\note{HS: not updated other baselines yet} Simulation results for CSP ($K=6$). 
  Figure~\ref{fig:k6n50} and Figure~\ref{fig:k6n200} show learning curves of each setting when $N=50, 200$ respectively. 
  There are 2500 training steps in an episode.
  Figure~\ref{fig:HeurvsPsharing} compares reward curves of two different algorithms which consider future transition after selection or not.} 
  \label{fig:K6}
\end{figure*}


\begin{figure*}[ht]
  \centering
  \subfloat[$N=10, K=4$ \label{fig:K4N10} ]{\includegraphics[width=0.265\textwidth]{figure/pp_K-4_conf-graph_ne-10.pdf}}
  \subfloat[$N=10, K=7$\label{fig:K7N10}]{\includegraphics[width=0.265\textwidth]{figure/pp_K-7_conf-graph_ne-10.pdf}} 
  \subfloat[$N=10, K=10$\label{fig:K10N10}]{\includegraphics[width=0.265\textwidth]{figure/pp_K-10_conf-graph_ne-10.pdf}}
  \subfloat[$N=4, K=2$\label{fig:K2N4}]{\includegraphics[width=0.185\textwidth]{figure/circle_scenario}} 
  \caption{Figure~\ref{fig:K4N10},\ref{fig:K7N10},\ref{fig:K10N10} are learning curves for PP with $N=10$ predators, 4 preys, and $K=4,7,10$, respectively. 
  Each episode consists of 175 steps. 
  Figure~\ref{fig:K2N4} describes some examples when 
  there exist $N=4,K=2$ with 4 preys in a $6 \times 6$ grid world. 
  The trained Q-network $Q_{1}$ acts green or sky shaded and black lined arrow after it observes the different p-states $s_{1}$ which are denoted as the same colored shaded arrow.
 \note{goes to analysis: No matter what $Q_{0}$ selects, the $Q_{1}$ tries to select proper a predator and a command near the selected predator since a prey should be caught simultaneously by more than two predators.} 
}
  \label{fig:predator-prey}
\end{figure*}


\subsection{Multiple Item Selection ($K>1$)}
To check the performance of ISQ with multiple cascaded Q-networks, we test 3 versions of ISQ and the other baselines in CS and PP under varying $N$ and $K$.
To exploit the symmetry, we apply intra-parameter sharing to the whole baselines. 
In Figure~\ref{fig:K6}, we evluate the algorithms in CS with $K=6, |\mathcal{C}| = 5$, $U=0$ while $N=50,200$. 
In Figure~\ref{fig:predator-prey}, we test the algorithms in PP with  
 $10$ predators ($N=10$) and $4$ preys in a $10 \times 10$ grid world
while $K=4,7,10$.

The learning curves in both CS (Figure 7) and  PP (Figure 8) well illustrate ISQ outperforms the other baselines in most of the tasks even though we modify the baselines by adding I-shared Q-networks.
This fact strongly shows that ISQ successfully learns proper combinatorial effects of selected items in different large scale environments: CS and PP.
In the following parts, we will explain the specific advantages of ISQ.   
% \smallskip \noindent {\bf Impact of ISQ}
\subsubsection{Power of ISQ: Proper Selection}
Compared to ISQ, IDQN performs poorly in overall tasks, especially in CS. 
The reason is that SELECT-MDP is non-stationary to a single item’s perspective since the reward dramatically depends on the other selected items and their commands, especially in CS (zero rewards if collisions occur).
This non-stationary issue is alleviated a lot but still not solved although we use I-shared Q-networks. 
In RSQ cases, it performs very worse than ISQ when $K<<N$ whether CS or PP since there RSQ only focuses on allocates proper commands but not selects good items.
However, as $K/N$ grows to $1$, the gap between RSQ and ISQ decreases which shows that the importance of the selection relieves since most of the items are selected.  
In a MARL case when $K=N=10$ in Figure~\ref{fig:K10N10}, RSQ and ISQ show almost the same performance since the agent needs to focus on choosing a proper command for a selected item. 

In Figure~\ref{fig:k6n50}, \ref{fig:k6n200}, original ISQ ($\vert \cC \vert = 5$) outperforms ISQ-(1) ($\vert \cC \vert = 1$) during the entire training stage. 
This result is non-trivial since additional commands increase the action space by $\vert \cC \vert^K$ times compared to ISQ-(1) which make exploration with RL much harder. 
To sum up, ISQ shows its ability to exploit this large action space. 

Figure~\ref{fig:K2N4} shows some scenario how the $Q_{1}$ selects an item and a command for phase $1$ after observes two different p-state $s_{1}$ in PP. Details are explained in the caption.
%%0214 previous
% IDQN performs badly in overall tasks, especially in CS.
% The reason is that the selectable circles with large radius tend to have large expected values but large selectable circles easily collide each other so the reward becomes zero. 
% This denotes the problem of the independent selection by IDQN of items without considering other selected items. 
% In RSQ cases, bad performance is very natural when $K<<N$ whether CS or PP since the items are selected uniform randomly and the agent only chooses commands for selected items.
% However, as the $K/N$ grows, the gap between RSQ and ISQ decreases since the impact of the selection would decrease as most of the items would be selected. 
% In Figure 8c, a typical MARL case such as K=N, RSQ, and ISQ shows almost the same performance since the agent just needs to focus to choose a proper command for selected items. 

% In Figure~7a, 7b, ISQ with 5 commands outperforms than ISQ-I (1) during the entire training stage. 
% This result is non-trivial since additional commands increase the action space by $|\cC|^{K}$ times compared to ISQ (1) and make exploration much harder.
% However, ISQ’s Intra-shared structure makes possible to explore the much larger action space efficiently.

\subsubsection{Power of ISQ: Long-Term Reward Maximization}
Myopic Q-learning shows worse performance than ISQ
Figure~\ref{fig:HeurvsPsharing} represents distributions of the radius of circles selected by various algorithms during episodes when $N=200$. 
The radiuses of selected circles by ISQ are mainly distributed at both ends: very small or large. 
This strategy is pretty good since the circles grow very slowly with a constant but the reward is proportional to the area of the circle.
Therefore, the agent should wait until the middle-size circles grow enough although it sometimes selects tiny circles which does not matter whether it is regenerated with a small radius.
In contrast, MQ selects lots of middle size circles before grown up since MQ focuses on maximizing the myopic reward. 
Furthermore, RSQ and IDQN also select many middle size circles since they do not consider smart selection. 
   

% \smallskip \noindent {\bf Impact of inter parameter-sharing}
\subsubsection{Impact of inter-parameter sharing}
% In this part, we check the impact of inter-parameter sharing among different cascaded Q-networks which 
In this part, we analyze the impact of P-sharing among different cascaded Q-networks by comparing the learning curves of 3 types of ISQs: ISQ, ISQ-U, ISQ-P.
In ISQ-P or ISQ-U, each cascaded Q-networks $Q_{k}$ not only uses experience from its phase $k$ but also use experiences from the other phases $k'$ to train $Q_{k}$.
Therefore,  
 ISQ-P learns significantly faster than ISQ in all cases as well described by the learning curves in Figure \ref{fig:K6} and \ref{fig:predator-prey}. 
Furthermore, ISQ-U also shows comparable performances both in CS and PP even if the Q-networks are tied together during the whole training. 
Therefore, we can say that ISQ-P is also robust 
\note{HS: I want to write that ISQ-P is very robust to the time step that we differentiate the networks since ISQ-U show good performance… so whenever the networks are differentiated it would works}

% 02/13 erase
% The gap between our DQNs and the rule-based heursitic originates from the consideration of the next state after the combinatorial selection. 
% In CSP, the grow rate of the selectable circles are constant but pretty slowly.
% Therefore, the agent sometimes need to wait until radius of a circle increases enough.  
% However, the heuristic is myophic as it performs very well at the early stage by greedily exploiting all the largest circles.
% Therefore, eventually, there are no remaining large-sized circles so the performance decreases drastically.   
% In contrast, our ISQs are able to consider the future state transition. 
% This result is well represented in Figure~\ref{fig:HeurvsPsharing}. 



% \smallskip\noindent {\bf Generalization capability of ISQ} 
\subsubsection{Power of ISQ: Generalization capability}
\begin{table}
  \small
  \centering
  \subfloat[Circle Selection\label{table:inductive_CS}]{%
    % \hspace{.5cm}%
    \begin{tabular}{@{}c|cc@{}}
      \toprule
      \diagbox{$N_{tr}$ }{$N_{te}$} & $50$ & $200$ \\ \midrule
      \multicolumn{1}{l|}{$50$} & $1.00$ & $1.03$ 
      \\
      \multicolumn{1}{l|}{$200$} & $0.86$ & $1.00$ \\ \bottomrule
    \end{tabular}
    \hspace{.5cm}%
  } 
  % \hspace{1cm}
  \subfloat[Selective Predator-Prey\label{table:inductive_PP}]{%
    % \hspace{.5cm}%
    \begin{tabular}{@{}c|cc@{}}
      \toprule
      \diagbox{$N_{tr}$ }{$N_{te}$} & $4$ & $10$ \\ \midrule
      \multicolumn{1}{l|}{$4$} & $1.00$ & $0.95$ 
      \\
      \multicolumn{1}{l|}{$10$} & $0.76$ & $1.00$ \\ \bottomrule
    \end{tabular}
    % \hspace{.5cm}%
  }
  \caption{The normalized performance results for inductive applications of P-sharing. 
  $N_{tr}$ denotes the number of items during training while $N_{tr}$ denotes the number of items for test. The values are normalized so the performance equals to 1 whenever $N_{tr} = N_{te}$. }
  \label{table:inductive}
\end{table}
% The agent can save tremendous memory from parameter sharing of Q-networks. 
%   Table~\ref{table:memory} shows the required memory for the Q-Networks that are actually tested for  U-sharing, I-sharing, P-sharing and vanilla DQNs. 
  Another advantage of ISQ is powerful generality under different environments with different number of items. 
  This is very  important from a practical point of view since the number of the possible candidates can be varied very easily in real situation. 
  Normally, typical Q-network should be trained again whenever number of item sizes from training and testing are different.
  However, as aforementioned in Section~\ref{sec:EINET}, Q-networks with parameter sharing have the same number of weight parameters for different item sizes $N$. 
  Therefore, we can just re-use the trained parameter set for specific item size $N_{tr}$ to re-construct differernt Q-network to test with different item size $N_{te}$. 

  Table~\ref{table:inductive} shows the relative performances of ISQ-P with varying $N_{tr}$ and $N_{te}$ in CS and PP. 
  In Table~\ref{table:inductive_CS}, ISQ-P performs very well on different CS environments which they are not trained ($N_{tr} \neq N_{te}$) enough get a similar performances when $N_{tr} = N_{te}$ although there are fourfold difference between the numbers of the items. 
  Note that, the performance result when $N_{tr}=50, N_{te}=200$ is slightly better than the performance result when $N_{tr}=N_{te}=200$. 
  We conjecture that ISQ is able to learn a policy efficiently in an environment with small number of items and the trained knowledge is competitive to a different and more difficult environment with large number of items.
  We guess this fact is quite similar to human beings when they learn a policy for SELECT-MDP. 
  Table~\ref{table:inductive_PP} also shows this kind of generalization power in PP.  

\vspace{1cm}





%   \begin{table}
%     \centering
%     % \begin{tabular}{@{}c|ccc@{}}
%     \begin{tabular}{@{}c|cc@{}}
%       \toprule
%       \diagbox{DQN}{$N$} & $50$ & $200$ \\ \midrule
%       \multicolumn{1}{l|}{I-sharing} & $46.1$  &  $46.1$  
%       \\
%       \multicolumn{1}{l|}{U-sharing} & $18.4$  & $18.4$    \\
%       \multicolumn{1}{l|}{P-sharing} & $46.1$  &  $46.1$   \\
%       \multicolumn{1}{l|}{Vanilla} & $1.1\cdot10^{5}$ & $9.3\cdot 10^7$ \\ \bottomrule
%     \end{tabular}
%     \caption{\note{HS: prob goes to appendix} Requirement memory (kilobyte) for various Q-Networks for Sequential Circle Selection with $K=6$ and $\vert \cC \vert =5$. We do not trained vanillar Q-network in reality. As a number $N$ of items increases, the required memory for vanilla q-network drastically increases.}
%     \label{table:memory}
%   \end{table}
  


  
%   \begin{table}
%     \centering
%   \begin{tabular}{@{}c|cc@{}}
%     \toprule
%     \diagbox{$N_{tr}$ }{$N_{te}$} & $50$ & $200$ \\ \midrule
%     \multicolumn{1}{l|}{$50$} & $\mathbf{1.00}$ & $\mathbf{1.03}$ 
%     \\
%     \multicolumn{1}{l|}{$200$} & $0.86$ & $1.00$ \\ \bottomrule
%   \end{tabular}
%   \caption{Inductive application of ISQ when the numbers of items for training $N_{tr}$ and testing $N_{te}$ are different. 
%   The performance ratios  are normalized  to make  $1.00$ when $N_{tr} = N_{te}$.
%   }
%   \label{table:inductive}
%   % \end{table}
%   \end{table}


% \begin{figure}[ht] 
% \centering
% \includegraphics[width=\linewidth]{figure/Prey}
% \caption{Comparison of the inter-parameter sharing method with rule-based heuristic. The performances of ISQ for each $N $s are normalized with respect to the performance of the rule-based heuristics corresponding $N$. The result shows that ISQs outperform the heuristic for all $N$s.}
% \label{fig:pred-prey-learning}
% \end{figure}

% \paragraph{Environment: Predator-Prey} 

% \subsection{Selective Predator-Prey}
% \label{sec:Predator-Prey}
% In this task, there are multiple predators who should capture randomly moving preys. 
% The agent observes the positions of the  predators and preys in a 2-dimensional grid world.
% The agent selects $K$ predators and allocates one of the 5 commands to each predator: \textit{`stay', `up', `right', `left', `down'}.   
% The only selected predators are able to move and capture the preys. 
% The positive reward is given if and only if two or more predators catch a prey simultaneously. 
% The performance metric is the number of time steps taken to capture a prey. 
% In our experiment, there exist $N=10$ predators and 4 preys in a $10 \times 10$ grid world.
% We conduct the experiment with various $K=4,7,10$. 
% Note that, when $N=K=10$, this setting conincides to a fully cooperative multi-agent reinforcement learning problem which the other baselines originally intend to solve. 


% % In the select-MDP, predators are selectable elements and preys are unselectable elements.
% % (\note{HS: just explain the agent can moves predators})


% % Being initialized with a negative reward of $-0.005$,
% % the agent gets penalty of $0.01$ when one of the predators moves out of the map,
% % which is bounded in $[-1,1]$ interval.
% % When distance between a prey and a predator is less than a predefined value $d$,
% % the prey is caught, a new one is generated,
% % and the agent receives a positive reward $r_1=0.05$.
% % However, when distances from the prey to at least two predators are less than $d$,
% % a positive reward $r_2=0.5$ is given.
% % This scenario shows the complex combinatorial rule of our environment,
% % as it requires at least two predators to move towards a prey in the same time step.
% % In the environment, only selected predators can catch the prey.
% % Therefore, we set $d$ to $0.3$, which is pretty large,
% % because the given reward becomes too sparse to learn with smaller $d$.
% % % See more details about the environment in the Appendix \note{ref}.



% To compare with the inter-parameter sharing method,
% we designed a rule-based heuristic for predator-prey environment.
% The algorithm first calculates the distances from each predator
% to its closest prey, then gets $K$ smallest values among them.
% $K$ predators corresponding to these $K$ smallest distances are the selected ones.
% Finally, it makes the $K$ selected predators move towards their closest preys.
% The DQN with only I-sharing is not considered in this experiment, as it shows slow convergence in the Sequential Circle Selection, which is less complex than Predator-Prey.

% We conduct the experiment with number of predators $N = 20, 50, 100, 200$,
% while number of preys is fixed to $5$ and number of selections $K$ is fixed to $2$.
% As shown in Figure~\ref{fig:predator-prey}, 
% our inter-parameter sharing method performs better than the rule-based heuristic in all cases.
% Especially with larger number of predators as $N=100, 200$,
% the performances of ISQ are twice as much as the performances of the rule-based heuristic.
% This shows that ISQ correctly learns the combinatorial rule of sequential actions with commands,
% learns to move appropriate predators to a proper prey to achieve much higher reward.
% The main reason that the ISQ works better than the rule based algorithm is that ISQ is able to learn the combinatorial cooperation of the predators that catch the prey at once while the rule based algorithm just catch nearest prey so there is no consideration of the cooperation of the predators.  
% % which rule-based heuristic does not.
% % \note{check}


% % \begin{itemize}[\textcolor{red}{\textbullet}]
% % \item Simulation for $K=4$
% %   \begin{itemize}[\textcolor{red}{\textbullet}]
% %     \item settings: $N=5, 10, 20, 50$
% %     \item base algorithms: shared q-networks, greedy heuristic, (if possible iql with top $K$ selction)
% %     \item Goal: EINET can work well with various commands problem
% %     \item einet consider the combination effects of the sequential actions. (show with the real state examples)
% %     \item (if possible) EINET performs better than other independent q-learning with naive top $K$ selection.
% %   \end{itemize}
% % \end{itemize}

% % \note{HS: write the whole hyper parameter settings network + environment (again) with table in the appendixs. Refer the other RL papers. }





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> model_bk.tex <==
\section{Preliminary}
 \label{sec:model}

\begin{comment}
In this section, we introduce an equivalent conversion of select-MDP called greedy select-MDP.  We also define a special symmetry called the \textit{permutation equi-invariant (EI) property} in optimal q-values for the greedy select-MDP. 
The detailed definition of select-MDP $\cM:=\langle \cS, \cA, \cP, R, \gamma \rangle$ and the same polices are described in the appendix \ref{sec:select-MDP}. 
\end{comment}


\begin{comment}
\subsection{Select-MDP}
\label{sec:select-mdp}
To model a problem of sequentially selecting a set of $K$ ones in $N$ elements, we consider an MDP, which we call select-MDP (simply S-MDP) $M(K,N)$, described as a tuple $\langle S, A, P, R, \gamma \rangle$ associated with selecting $K$ items among the set $N$ items in $\set{N}=\{1, 2, \ldots, N \}$ and their corresponding commands in \set{C}. We assume that the available set of commands is the same across all items for simplicity. 
The state $s = \{i_1,\ldots,i_N\} \in S$ is a set of items' context, where $i_n \in S$ is the context of item $n \in \cN=\{1,\cdots, N \}$, with $|S|$ being finite. 
Each action $a = \{(n_1,c_1), \ldots, (n_K,c_K) \} \in \cA$ is a set of $K$ (item, command) pairs, 
% where the agent selects a set $\{n_1,\ldots,n_K\}$ of $K$ distinct items and assigns a command $c_k \in \set{C}$ for the selected item $n_k$. When action $a$ is played in state $s$, 
transition to a new state $s'$ occurs with probability $P(s'\mid s,a)$, and the agent receives reward $R(s,a)$ from action $a$ at state $s$. $\gamma \in [0,1]$ is the discount factor.
We consider the case when both of state observation and selection of $K$ elements are made simultaneously, implying that 
each state and action is a set, and thus they are permutation-invariant. 
\end{comment}
% \vspace{-0.05cm}
\subsection{Definition: Iterative Select-MDP (IS-MDP)}
\label{sec:greedy-mdp}
\begin{figure}
\subfloat[Select MDP (S-MDP)]{\includegraphics[width=0.99\linewidth]{figure/smdp_0223}}
\vspace{-0.4cm}
\subfloat[Iterative Select MDP (IS-MDP)]{\includegraphics[width=0.99\linewidth]{figure/ismdp_0223}}
\vspace{-0.3cm}
  \caption{ 
    Example of a S-MDP and its associated IS-MDP when $N=3,K=2$.
    %  An action $\tilde{a} = \{(i_2,c_1),(i_3,c_2)\}$ in S-MDP is divided into $2$ phases of actions $a=(i_2,c_1)$ and $a=(i_3,c_2)$ in IS-MDP.
    %: in the first phase, the action $a_1 = (2,c_1)$ is taken; the deterministic transition occurs with zero reward; and in the second phase the action $a_2 = (3,c_2)$ is taken.
   }  
   \label{fig:MDPs}
\vspace{-0.25cm}
  \end{figure}
In this section, we will introduce the formal definition of IS-MDP $\cM=\langle \tcS, \tcA, \tcP, \tcR, \tgam \rangle$ which is an divided version of S-MDP.
Recall that 
in IS-MDP, the agent iteratively selects each item (and its command) one by one through $K$ divided steps  and receives reward $\tilde{r}$ after $K$ actions. 
Figure~\ref{fig:MDPs} describes the relationship between S-MDP and IS-MDP.
% Thus, IS-MDP turns out to learn its policy with a smaller number of actions per state, but with a larger state space. 
% Fron now on this paper, we only deal with IS-MDP. 
% We formally describe IS-MDP$(K,N)$ as a tuple $\langle \tcS, \tcA, \tcP, \tcR, \tgam \rangle$
% \footnote{We use different fonts to differentiate two MDPs: upper-case times-roman and caligraphic fonts for S-MDP and IS-MDP, respectively. However, most of our presentation in this paper is focused on IS-MDP.},

\smallskip\noindent{\bf{State space.}}
% Before describe the state space, let us first define some concepts already described in Section~\ref{sec:intro}.
Let $i_{n} \in \cI $ as information  and $c_{n} \in \cC$ as command of item $n$ for $1 \leq n \leq N$ where
$\cI$ and $\cC$ are the information space and the command space respectively. 
Note that $C=\vert \cC \vert$. 
For the selection of the $(k+1)$th item, the agent observes (information, command) of the $k$ already selected items but only information of the remained items.
Therefore, there are $K$ types of state depend on phase $k$ in the overall state space $\cS$, i.e., 
 $\cS := \dot \bigcup_{0 \leq k < K} \cS_{k}$ where
% $\cS_{k}$ denotes the state space when the agent select the $k$th item.
% $$\cS_{k}:=\{ ((i_{1}, c_{1}), \cdots, (i_{k-1},c_{k-1})), ((i_{k}, \cdots, i_{N}) ) \}. $$
$$\cS_{k}:=\{ (x_{1}, \cdots,x_{k}), (i_{1}, \cdots, i_{N-k}) \, \vert \, x \in \cI \times \cC , i \in \cI \}.  $$
% Note that $x_{j} = (i_{j},c_{j}) \in \cX$ ($:=\cI \times \cC$) represents for the selected item $j$'s (information, command) pair.
To summarize, for the $k$th selection, the agent observes  a state $s =(\bx, \bi)$ where $\bx:= (x_{1}, \cdots,x_{k}) \in (\cI \otimes \cC)^{k}$ and $\bi:=(i_{1}, \cdots, i_{N-k}) \in \cI^{N-k}$. 
Denote $\cX:=\cI \otimes \cC$ for notational convenience.  
Note that $\cS_{k}=\cX^{k}\otimes \cI^{N-k}$ and the aforementioned state $\tilde{s}=(\bi)=((i_{1}, \cdots, i_{N}))$ in S-MDP belongs to $\cS_{0}$.  

\smallskip \noindent {\bf Action space:} $\cA(s)$.
After the agent observes a state $s$ at phase $k$, the agent selects an item among the $N-k$ remained items $\bi = (i_{1}, \cdots, i_{N-k})$. 
Similar to $\cS$, the action space $\cA(s)$ for the state $s=(\bx,\bi)$, 
% = \bigcup_{0 \leq k < K} \cA_{k}$ where 
\begin{equation} \label{eq:action space}
\cA(s):= \{(i, c) \, \vert \, i \in \bi, \, c \in \cC \}.
\end{equation}
It is easy to see that the number of possible actions for the state $s$ also depends on  the phase $k$ which $s$ belongs to. 

\smallskip  \noindent { \bf Transition probability function.} 
In IS-MDP, the agent recieves a deterministic state transition with zero reward  in the first $(K-1)$ phases and
 receives the probabilistic transition of S-MDP at phase $K-1$.  
 \begin{align}
  \label{eq:EQUIGreedyTran}
  \begin{split}
  & k<K-1, \quad \cP(s', 0 \mid s,a) \equiv 1, \\
  & k=K-1, \quad \cP(\tilde{s}', \tilde{r} \mid s, a) \equiv \tilde{\cP}(\tilde{s}', \tilde{r} \mid \tilde{s}, \tilde{a}), 
  \end{split}
  \end{align}
  where $s = (\bx, \bi)$, $a=(i,c)$, $s' = (\bx + (i,c), \bi - i)$ \footnote{Note that we abuse  $+,-$ as  $\bx + x:=(x_{1}, \cdots, x_{k}, x)$ and $\bi - i$ is a tuple which the element $i$ is removed. }
 and 
 $\tilde{\cP}(\tilde{s}', \tilde{r} \mid \tilde{s}, \tilde{a})$ is the transition probability function of in S-MDP corresponding to $K$ steps in IS-MDP (Section~\ref{sec:intro}). 
 
 It is proven that this kind of IS-MDP and S-MDP are equivalent in that the optimal policy for IS-MDP can be directly applied to S-MDP and vice versa  \cite{maes2009structured}.  
Therefore, our algorithm focuses on IS-MDP only.


% \vspace{-0.05cm}
\subsection{Deep Q-network (DQN)}
We provide a background of DQN \cite{mnih2015human} which is known for a base-line deep RL algorithm.
The goal of a standard RL approach based on an MDP is to learn an optimal policy %$\pi(a|s): \cS \mapsto \cA$
$\pi^{\star}(a|s): \cS \times \cA \mapsto [0,1]$ that maximizes the expected discounted return. 
We denote the optimal action-value functions (Q-function) under the optimal policy $\pi^{\star}$ by $Q^{\star}(s,a)$.
% The equivalence of the optimal policies of the original S-MDP and the associated IS-MDP has been studied in \citet{maes2009structured}.
Deep Q-network (DQN) parameterizes an approximate the optimal Q-function $Q^{\star}(s,a)$ using the so-called Q-network $Q(s,a; \omega)$, i.e., a deep neural network with a weight parameter vector $\omega$. In DQN, the parameter $\omega$ is learnt by sampling minibatches of experience $\be = (s,a,r,s')$ 
% i.e., either $(s_k,a_k,0,s_{k+1})$ for $0 \leq k < K-1$  or $(s_{K-1},a_{K-1},r,s'_0)$ in our IS-MDP, 
from the replay memory and using the following loss function:
\begin{align} \label{eq:loss_general}
  %l(\ts, \ta, r, \ts ' ; \omega):= (\tQ(\ts,\ta;\omega) - (r+\tgam \max_{\ta ' \in \tcA(\ts)}  \tQ(\ts ',\ta;\omega ')))^{2},
  l_{\be}(\omega) = \Big(\tQ(\ts,\ta;\omega) - \large(r+\tgam \max_{\ta ' \in \cA(s')}  \tQ(\ts ',\ta';\omega ') \large)  \Big)^{2}
\end{align}
where $\omega'$ is the target parameter which follow the main parameter slowly. In implementing a DQN, it is common to approximate $\tQ(\ts;\omega):\tcS \rightarrow \Real^{\tcA(\ts)}$ rather than $\tQ(\ts, \ta;\omega)$ using a neural network due to easy computation of all action values at once.
% The targer parameters $\omega'$ is only updated with $\omega$ every a certain steps, and is held fixed between individual updates: description from DQN paper.

\iffalse 02/23
\subsection{Iterative Select-MDP (IS-MDP)}
\label{sec:greedy-mdp}

\begin{figure}   \label{fig:MDPs}
\subfloat[Select MDP (S-MDP)]{\includegraphics[width=0.99\linewidth]{figure/smdp}}
\vspace{-0.4cm}
\subfloat[Iterative Select MDP]{\includegraphics[width=0.99\linewidth]{figure/ismdp}}
\vspace{-0.2cm}
  \caption{ 
    Example of a S-MDP and its associated IS-MDP when $N=3,K=2$. An action $\tilde{a} = \{(i_2,c_1),(i_3,c_2)\}$ in S-MDP is divided into $2$ phases of sequentially choosing pairs of $a=(item,command)$ in IS-MDP.
    %: in the first phase, the action $a_1 = (2,c_1)$ is taken; the deterministic transition occurs with zero reward; and in the second phase the action $a_2 = (3,c_2)$ is taken.
   }  
\end{figure}


Given a S-MDP$(N,K)$ as described Section~\ref{sec:intro}, 
we consider a modified MDP from the original S-MDP, called Iterative Select-MDP (simply IS-MDP), which iteratively selects each item (and its command) one by one through $K$ phases rather than selecting $K$ items and commands all at once. Thus, IS-MDP turns out to learn its policy with a smaller number of actions per state, but with a larger state space. We formally describe IS-MDP$(K,N)$ as a tuple $\langle \tcS, \tcA, \tcP, \tcR, \tgam \rangle$
\footnote{We use different fonts to differentiate two MDPs: upper-case times-roman and caligraphic fonts for S-MDP and IS-MDP, respectively. However, most of our presentation in this paper is focused on IS-MDP.},
 where $\cS = \cup_{0 \le k < K } \cS_{k}$ and $\cA = \cup_{0 \le k < K} \cA_k$ are state space and action space, respectively. Having $k$-th (item, command) selection as an action in each {\em $k$ phase}, the agent observes the state
%$s_k = (\bx, \by) \in \cS_k$, 
$s_k = ( \{x_1,\ldots,x_k\},  \{y_1,\ldots,y_{N-k}\} ) \in \cS_k $, 
as a set of the $k$-item informations and their commands, selected during the prior phases, and a set of the informations of $N-k$ unselected items, i.e., $x_j = (i_{n_j},c_j)$ is defined from the selection of item $n_j$ and command $c_j$ in prior phases, and $y_j = i_{n_j}$ is the information of the unselected item $n_j$. Then, the action space of \textit{phase-state} (p-state) $s_k$ is given by $\cA_k(s_k) = \{ (i,c) \mid i \in \{ y_1,\ldots,y_{N-k}\}, c \in \cC \}$. The transition to a p-state in next phase is defined as: for $s,s' \in S$ and $a \in A$ in the original S-MDP $\langle S,A,P,R,\gamma \rangle$,  
\begin{align}
\label{eq:EQUIGreedyTran}
\begin{split}
& k<K-1, \quad \cP(\ts_{k+1}, 0 \mid \ts_{k}, \ta_{k}) \equiv 1, \\
& k=K-1, \quad \cP(s_0', r \mid \ts_{k}, \ta_{k}) \equiv P(\tilde{s}', \tilde{r} \mid \tilde{s}, \tilde{a}), 
\end{split}
\end{align}
i.e., the transitions in the first $k-1$ phases, given per-phase action (p-action)$a_{k}$, are deterministic with zero reward, while the transition in the final p-state $s_{K-1}$ to the $0$th phase of a new p-state $s'$ occurs with transition probability $P$ of the original S-MDP, followed by the corresponding reward. Note that we just use the word as p-state $s_{k}$ and p-action $a_{k}$ for convenience to compare easily with the state $s$ and action $a$ in S-MDP but $s_{k}$ and $a_{k}$ are just state and action by the definition for IS-MDP. See Figure~\ref{fig:MDPs} to illustrate an example of IS-MDP.
\fi

\begin{comment}
Jointly inferring the $K$ pairs of (item, command) incurs high complexity. For this reason, we consider a modified MDP from the original S-MDP, called Iterative Select-MDP (simply IS-MDP), which iteratively selects each item one by one rather than selecting $K$ items (and their commands) all at once. Thus, IS-MDP turns out learn a policy in the MDP with a smaller number of actions per state, but with a larger state space. We formally describe IS-MDP by $\cM(K,N)= \langle \tcS, \tcA, \tcR, \tcP, \tgam \rangle.$ \footnote{We use different fonts to differentiate two MDPs: upper-case times-roman and caligraphic fonts for S-MDP and IS-MDP, respectively. However, most of our presentation in this paper is focused on IS-MDP.} 
% where $\tcS, \tcA, \tcR, \tcP, \tgam$ denote the state spaces, action spaces, reward function, transition probability, and discount factor.
% In greedy select-MDP, the agent iteratively selects a single item $n_{k}$ and its corresponding command $c_{k}$ per each step, rather than selecting $K$ items and commands all at once. 
% This modification helps to remove the complexity of inferring joint selections and commands while increases the complexity of the state space.
% In the further section \ref{sec:Methods}, we describe how we handle this complex state space with our parameter neural network arhictectures.
% To consider the combination effects of the previously selected items and commands $\{(n_{1}, c_{1}), \cdots, (n_{k-1}, c_{k-1}) \}$, the agent adds this informations to state $\ts$. 
The state space $\tcS=\cup_{0 \le k < K } \cS_{k},$ where $\cS_k$ is the set of spaces of {\em $k$ phase,} 
corresponding to a state where $k$ pairs of (item, command) has already been selected, having $k$-th (item,command) selection as an action, (\note{HS: can we say 0th action $a_{0}:=(1,c)$ when $k=0$? or we need to say $1$th action for state $s_{0}$?}) i.e.,   
$ \tcS_k =  \Big \{ (\{x_1, \ldots, x_k\} \cup \{ \{ y_1, \ldots, y_{N-k} \} \otimes \cC \}) \Big\},$ where $x_j$, $y_j$ are the pairs of selected items' (context, command) or unselected items' contexts, respectively. Similarly, the action space $\cA$ can be defined by each phase, $\cA = \cup \cA_k$, where $\cA_k$ is the set of actions that are available at phase $k,$ i.e., for state $s_k = (\{x_1, \ldots, x_k\} \cup \{ y_1, \ldots, y_{N-k} \}),$ we have that $\cA_{k} = \{(i,c) \mid (i,c) \in \{y_1, \ldots, y_{N-k}\} \otimes \cC \}.$ We henceforth use state $s_k$ and action $a_k$ to refer to a state and an action at phase $k.$ 
Then, the transition probability $\tcP$ of IS-MDP is such that: for two states $s,s' \in S$ in the original S-MDP, 
\begin{align}
\label{eq:tranGREEDYSEL}
\begin{cases}
\cP(\ts_{k+1}, 0 \mid \ts_{k}, \ta_{k}) \equiv 1, & \text{if} \quad k  \in \{ 0,\cdots, K-2 \},\cr
\cP(s', r \mid \ts_{K-1}, \ta_{K-1})) \equiv P(s', r \mid s, a), & \text{if} \quad k = K-1, 
\end{cases}
\end{align}
where recall that $P$ is the transition probability in the original S-MDP. During the transitions prior to finally select $k$-th pair of (item, command), given a per-phase action, they are deterministic with zero reward. See Figure~\ref{fig:MDPs} to illustrate an IS-MDP.


\begin{figure*}[ht]  
  \begin{subfloat}{1\textwidth}
    \centering
    \begin{minipage}{1\textwidth}
      \includegraphics[width=\linewidth]{figure/smdp}
      \vspace{-1.5cm}
       \subcaption{\bf{Select-MDP}}
    \end{minipage}
    \begin{minipage}{1\textwidth}
      \vspace{0.5cm}
      \includegraphics[width=\linewidth]{figure/ismdp}
      \subcaption{\bf{Iterative Select-MDP}}
    \end{minipage}
  \end{subfloat}
  \caption{Select-MDP vs Iterative Select-MDP. Compare an equivalent transitions in S-MDP and IS-MDP when $N=5,K=2$. One action $a=\{(2,c_{1}), (4,c_{2})\}$ is divided into $K$ phases in IS-MDP. The first action $a_{1}=(2,c_{1})$ implies the agent selects item $2$ and assigns command $c_{1}$. 
  During phase, the intermediate state $s_{1}$, the agent only gets reward as zero.
  The agent considers combination effect by considering   $\bx$ which implies the set of   (context, command) pairs for the selected items while $\by$ denotes the set of  contexts for unselected items.
   }
   \label{fig:MDPs}
\end{figure*}

As in the standard MDP, a policy $\pi(\ta | \ts): \cS \times \cA \rightarrow [0,1]$  is defined as the probability that the agent chooses action $\ta$ from state $\ts$. We denote by the state-value and the action-value functions by $\tV_{\pi}(\ts)$ and $\tQ_{\tpi}(\ts,\ta),$ respectively. 
It has been proved by \citet{maes2009structured} that a given S-MDP $M$ and its associated IS-MDP $\tcM$
shares optimality, meaning that the cumulative rewards from the optimal policies of $M$ and $\cM$ are equivalent. 
\end{comment}
\begin{comment}
In this subsection, we introduce an algorithm to solve Iterative Select-MDP based on Deep Q-Network (DQN) \citep{mnih2015human}.
DQN tries to approximate the optimal action-value function $\tQ^{\star}(\ts)$ with a deep neural network $\tQ(\ts; \omega)$ parameterised by $\omega$. 
For Iterative Select-MDP, a transition in Select-MDP is divided into $K$ phases as described in Figure~\ref{fig:MDPs}. 
It uses a replay memory to store these transitions like $(s_{k},a_{k}, 0, s_{k+1})$ for $0 \leq k < K-1$
or $(s_{K-1},a_{K-1}, r, s_{K})$.
The parameter $\omega$ is learnt by sampling batches of transitions from the replay memory and minimising the loss function $l(\omega)$,
\begin{align} \label{eq:loss_general}
  l(\ts, \ta, r, \ts ' ; \omega):= (\tQ(\ts,\ta;\omega) - (r+\tgam \max_{\ta ' \in \tcA(\ts)}  \tQ(\ts ',\ta;\omega ')))^{2},
\end{align}
where $\omega '$ denotes target parameter which is updated by following the main parameter $\omega$ during training.
\end{comment}

% are equivalent \cite{maes2009structured} and which means that the both optimal policy $\pi^{\star}(s)$ for $\cM$ and
%  $\tpi^{\star}(\ts_{0})$ for $\tcM$ has the same state value for all $s \in \cS$. 
% From now on, we focus only on greedy select-MDP and present  SELECT DQN to approximate the optimal $\tQ^{\star}(\ts, \ta)$. 



% The state-value function $\tV_{\tilde{\pi}}(\ts)$ is the expected reward sum from $\ts$ under $\tilde{\pi}$.
% Similarly, the action-value function $\tQ_{\tpi}(\ts,\ta)$ is defined as 
% $\tQ_{\tpi}(\ts,\ta):= \bE_{\ta \sim \tpi(\cdot | \ts)}[\tcR(\ts, \ta) + \tgam \tV_{\tpi}(\ts ')]$ where $\ts '$ denotes the next state for greedy select-MDP. 
% The goal of reinforcement learning is to find the optimal policy $\tpi^\star$ which maximizes  $\tV_{\tpi}(s)$ or  $\tQ_{\tpi}(\ts,\ta)$ over all policies. 
% It is proven that select-MDP $\cM$ and select-greedy MDP $\tcM$ are equivalent \cite{maes2009structured} and which means that the both optimal policy $\pi^{\star}(s)$ for $\cM$ and
%  $\tpi^{\star}(\ts_{0})$ for $\tcM$ has the same state value for all $s \in \cS$. 
% From now on, we focus only on greedy select-MDP and present  SELECT DQN to approximate the optimal $\tQ^{\star}(\ts, \ta)$. 

  


% in select-MDP. 
% Intermediate transitions ($k<K-1$) are deterministic with zero reward since these transitions are synthetic transitions that we defined. Intermediate transitions can also be regarded as internal transitions within the agent. 
% The difference between select-MDP and greedy select-MDP is illustrated in Figure~\ref{figure:mdp}.

% \begin{align} \label{eq:tranGREEDYSEL}
%   \begin{split}
%    k  \in \{ 0,\cdots, K-2 \}, \quad & \cP(\ts_{k+1}, 0 \mid \ts_{k}, \ta_{k}) \equiv 1 , \\
%     k = K-1, \quad & \cP(s', r \mid \ts_{K-1}, \ta_{K-1})) \equiv \cP(s', r \mid s, a)
%   \end{split}
% \end{align}
% where $\cP$ is the transition in select-MDP. 
% Intermediate transitions ($k<K-1$) are deterministic with zero reward since these transitions are synthetic transitions that we defined. Intermediate transitions can also be regarded as internal transitions within the agent. 
% The difference between select-MDP and greedy select-MDP is illustrated in Figure~\ref{figure:mdp}.

% $ \\\\ $
% $a = \{(i_{1}, c_{1}), \cdots, (i_{K}, c_{K}) \}$
% The agent considers the state $\ts_{k}:=(\{\tx_{1}, \cdots, \tx_{k}\})$ 
% An action $a=\{ (i_{1}, c_{1}), \cdots, (i_{K}, c_{K}) \} \in \cA$ in SELECT MDP is divided into sequential $K$ subactions $\ta_{k} := (i_{k}, c_{k})$ for $k=1, \cdots, K$ in SELECT-GREEDY MDP. 

% When the agent chooses $\ta_{k}$, the agent considers the state $\ts_{k}:=(s, \ta_{1..k-1})$ which implies that it considers both the current state $s \in \cS$ as well as history of $k-1$ subactions  $\ta_{1..k-1} := \{ (i_{1}, c_{1}), \cdots, (i_{k-1}, c_{k-1}) \}$.
% Since there are $K$ types of state $\ts_{k}$ for $k=1, \cdots, K$, 
% the total state space $\tcS:= \cup_{k=1}^{K} \tcS_{k}$ 
% is an union of $K$ sub-state spaces $\tcS_{k}:=\{ (\ts,  \ta_{1..k-1}) \mid  \ts \in  \cS, a \in \cA \}$. 
% For the given state $\ts_{k}$, the agent can selectes item $i_{k}$ among the remained item set $\tcI(\ts_{k}):= \cN \setminus \{i_{1}, \cdots, i_{k-1} \}$  and allocates command $c_{k}$ to the selected item $i_{k}$, i.e., the possible action set from state $\ts_{k}$,  $\tcA(\ts_{k}):= \tcI(\ts_{k}) \times \cC$. 
% The transition propbability $\tilde{\cP}$ in SELECT-GREEDY MDP is defined as 
% \begin{align} \label{eq:tranSELGREEDY}
%   \begin{split}
%    k  \in \{ 1,\cdots, K-1 \}, \quad & \tilde{\cP}(\ts_{k+1}, 0 \mid \ts_{k}, \ta_{k}) \equiv 1 , \\
%     k = K, \quad & \tilde{\cP}(s', r \mid \ts_{k}, \ta_{k})) \equiv \cP(s', r \mid s, a).
%   \end{split}
% \end{align}

% For $k\in \{1,\cdots, K-1\}$, $\tcP$ is deterministic  and intermediate which not exists in real SELECT MDP.
% During these transitions, the agent can not receive the reward $r$ from the environment, so we set $0$ as the intermediate reward.

% From the symmetry in \eqref{eq:select-mdp-pi}, $\tcP(\ts, \ta)$ defined in \eqref{eq:tranSELGREEDY} also satisfies below properties with the definition of $\sigma_{k}, \sigma_{N-k+1} $ belongs to the permutation $\cS_{k}$ and $\cS_{N-k+1}$, respectively.

% \smallskip\noindent{\bf Policy $\tilde{\pi}$ and Action-value function $\tilde{Q}_{\pi}(\tilde{\bs})$. } 






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> relatedwork.tex <==


